Optimal Auctions vs. Anonymous Pricing: Beyond Linear Utility

The revenue optimal mechanism for selling a single item to agents with independent but non-identically distributed values is complex for agents with linear utility (Myerson,1981) and has no closed-form characterization for agents with non-linear utility (cf. Alaei et al., 2012). Nonetheless, for linear utility agents satisfying a natural regularity property, Alaei et al. (2018) showed that simply posting an anonymous price is an e-approximation. We give a parameterization of the regularity property that extends to agents with non-linear utility and show that the approximation bound of anonymous pricing for regular agents approximately extends to agents that satisfy this approximate regularity property. We apply this approximation framework to prove that anonymous pricing is a constant approximation to the revenue optimal single-item auction for agents with public-budget utility, private-budget utility, and (a special case of) risk-averse utility.

==> Notes/PricingFunction.tex <==
\subsection{Allocation/Payment Characterization}

In this subsection, we introduce some 
characterization of the allocation rule and 
the
payment rule in the private-budget setting.
To clarify, we consider the setting where agents can overbid their budget as long as the payment does not
exceed the their true budget.

\begin{definition}
A mechanism ($\alloc, \price$) 
where 
the allocation rule $\alloc:V \times W \rightarrow [0,1]$, and
the payment rule $\price: V \times W \rightarrow \mathbb R^+$ 
is \emph{truthful} if for all types $(\val, \wealth)$,
$$
\begin{array}{rll}
\forall \val'\in V:
\quad
&\val\cdot \alloc(\val, \wealth) - \price(\val, \wealth)
\geq 
\val\cdot \alloc(\val', \wealth) - \price(\val', \wealth)
\quad 
&\text{(value-IC)}\\
\forall \wealth'\in W 
\text{ s.t. } \price(\val, \wealth') \leq \wealth:
&\val\cdot \alloc(\val, \wealth) - \price(\val, \wealth)
\geq 
\val\cdot \alloc(\val, \wealth') - \price(\val, \wealth')
&\text{(budget-IC)}\\
\end{array}
$$

\end{definition}

Same as the quasi-linear agents setting, the payment identity still holds for the private-budget setting.

\begin{lemma}
Given any truthful mechanism ($\alloc, \price$),
the allocation rule $\alloc$, and
the payment rule $\price$ 
satisfy that for all types $(\val, \wealth)$
$$
\price(\val, \wealth) = \val\cdot \alloc(\val, \wealth) - \int_0^\val \alloc(t, \wealth)dt.
$$
\end{lemma}
\begin{proof}
Using Myerson's argument for quasi-linear agents, value-IC is sufficient to uniquely 
pin-down the payment rule from the allocation rule.
\end{proof}

Next, we want to show that under mild assumption, the 
allocation $\alloc(\cdot, \bar\wealth)$ for agents with highest budget $\bar\wealth$, 
is sufficient to uniquely pin-down the allocation $\alloc(\cdot, \wealth)$
for agents with any budget $\wealth$.

\begin{assumption}\label{asp:right-continuous}
The allocation rule $\alloc(\val,\wealth)$ is 
\emph{right-continuous} in $\val$ every where.
\end{assumption}

\begin{lemma}\label{lem:price dominant}
Under \Cref{asp:right-continuous}, 
for any truthful mechanism ($\alloc, \price$),
for all types $(\val, \wealth)$,
$p(\val, \wealth) \leq p(\val,\bar\wealth)$.
\end{lemma}

\begin{proof}
We prove this lemma by contradiction. 
Suppose there exists some type $(\val, \wealth)$ such that
$p(\val, \wealth) > p(\val,\bar\wealth)$.
The budget-IC constraints between 
type $(\val, \wealth)$ and type $(\val, \bar\wealth)$
implies 
$$
\val\cdot \alloc(\val, \wealth) - \price(\val, \wealth)
=
\val\cdot \alloc(\val, \bar\wealth) - \price(\val, \bar\wealth).
$$ 
Combining with our assumption that $p(\val, \wealth) > p(\val,\bar\wealth)$, it implies
$$
\alloc(\val, \wealth) > \alloc(\val, \bar\wealth).
$$
This leads to the following contradiction. 
Notice that the value-IC constraint between the type 
$(\val+\epsilon, \bar\wealth)$ and the type $(\val,\wealth)$
for some sufficient small $\epsilon > 0$ is violated 
under \Cref{asp:right-continuous}, i.e., 
$$
(\val+\epsilon)\cdot \alloc(\val+\epsilon, \bar\wealth) - \price(\val+\epsilon, \bar\wealth)
<
(\val+\epsilon)\cdot \alloc(\val, \wealth) - \price(\val, \wealth).
$$
where the inequality holds since the derivative of the 
difference between the utility of truthful reporting and misreporting the
type $(\val, \wealth)$ at type $(\val, \bar\wealth)$ is 
$\alloc(\val, \bar\wealth) - \alloc(\val, \wealth) < 0$.
\end{proof}

\begin{corollary}\label{cor:allocation dominant}
Under \Cref{asp:right-continuous}, 
for any truthful mechanism ($\alloc, \price$),
for all types $(\val, \wealth)$,
$x(\val, \wealth) \leq x(\val,\bar\wealth)$.
\end{corollary}
\begin{proof}
It is directly implied by the budget-IC constraint
between 
type $(\val, \wealth)$ and type $(\val, \bar\wealth)$
and \Cref{lem:price dominant}.
\end{proof}

\begin{lemma}
%Under \Cref{asp:right-continuous},
Suppose $\alloc$ is continuous in $\val$,
for any truthful mechanism ($\alloc, \price$),
for all types $(\val, \wealth)$,
\begin{align*}
    \alloc(\val, \wealth) =
    %\left\{
    %\begin{array}{ll}
    %     \alloc(\val, \bar\wealth)  
    %     \quad&
    %     \text{if } \val \leq \val^*\\
    %     \alloc(\val^*, \bar\wealth) &
    %     \text{otherwise}
    %\end{array}
    %\right.
    \alloc(\min\{\val^*, \val\}, \bar\wealth) 
    %\quad 
    %\text{where  $v^*$ is the largest value such that
    %$\price(\val^*, \bar\wealth) \leq \wealth$}.
\end{align*}
where  $v^*$ is the largest value such that
$\price(\val^*, \bar\wealth) \leq \wealth$.
\end{lemma}
\begin{proof}
For all ``low-value'' types $(\val, \wealth)$ such that $\val \leq \val^*$,
the budget-IC constraint between type $(\val, \wealth)$ and type $(\val, \bar\wealth)$ implies
$$
\val\cdot \alloc(\val, \wealth) - \price(\val, \wealth)
=
\val\cdot \alloc(\val, \bar\wealth) - \price(\val, \bar\wealth).
$$
Combining with \Cref{cor:allocation dominant}, it implies 
$\alloc(\val, \wealth) = \alloc(\val, \bar\wealth)$.

For all ``high-value'' types $(\val, \wealth)$ such that $\val > \val^*$, due to the budget constraint and the allocation
for all ``low-value'' types pinned down above, 
it follows that $\alloc(\val, \wealth) = \alloc(\val^*, \bar\wealth)$.
\end{proof}
\begin{comment}
\begin{corollary}
Suppose there is no mass point in valuation space $V$, 
for any ex-ante constraint, 
it is W.L.O.G. to consider the pricing function 
which is continuous, increasing and convex.
\end{corollary}
\end{comment}

==> Paper/close_imply_regular.tex <==
\begin{tikzpicture}[scale = 0.5]
%\fill[gray!40!white] (0, 0) -- (8, 0) -- (8, 7) -- (0, 7);

\draw (-0.2,0) -- (15.2, 0);
\draw (0, -0.2) -- (0, 9.2);

\begin{scope}[very thick]

\draw [dotted] (6.7, 0) -- (6.7, 7.3);
\draw [dotted] (4.8, 0) -- (4.8, 4.8);
\draw [dotted] (3.4, 0) -- (3.4, 6.8);

\draw plot [smooth, tension=0.6] coordinates { (0,0) (2,6) (9, 7) (15,0)};

\draw [dashed] plot [smooth, tension=0.6] coordinates { (0,0) (1,3) (4, 5) (8, 3)  (12,1.6) (15,0)};
\draw (0, 0) -- (9, 9);
\draw (0, 0) -- (4.5, 9);

\end{scope}
\draw plot [smooth, tension=0.6] coordinates { (0,0) (2,3) (9, 3.5) (15,0)};

\draw (0, -0.8) node {$0$};
\draw (6.7, -0.8) node {$\sfrac{1}{\beta}$};
\draw (15, -0.8) node {$1$};

\draw (-0.6, 0) node {$0$};
\draw (-0.6, 9) node {$\revcurve$};
\draw (3.4, -0.8) node {$\exanteprobability$};
\draw (4.8, -0.8) node {$\correspondingquant$};
\draw (9.8, 9) node {$\sfrac{\exanteprice}{\alpha}$};
\draw (5, 9) node {$\exanteprice$};

\end{tikzpicture}



==> Paper/cover.tex <==
\vspace{10pt}
\begin{center}
{\huge Cover Letter}
\end{center}
\vspace{30pt}
\noindent Dear editors:
\newline
\newline
%\newline
\noindent We would like to submit our paper 
``Optimal Auctions vs.\ Anonymous Pricing: Beyond Linear Utility'' 
to Journal of Economic Theory. 
A two-page extended abstract of this paper has appeared at $20^{\text{th}}$ ACM conference on Economics and Computation (EC'19). 
This submission is part of the EC forward-to-journal process. 
Upon submission to JET, the EC'19 reviews will be forwarded, 
along with reviewer identities, to the contact editor (Alessandro Pavan). 

%\newli
In this submission, we have substantially improved the writing of the paper, 
and illustrated the connections between our assumptions on the closeness of the revenue curves. 
We improved our reduction framework to show tighter bounds for anonymous pricing 
when we have extra information about the gap
between the optimal ex ante revenue 
and optimal price posting revenue (Theorem 3.2). 
We also improved the upper bounds 
when agents have public budgets and regular valuation distributions (Theorem 4.1), 
which implies that when comparing the revenue of anonymous pricing to the ex ante relaxation, 
worst case happens when budgets never binds. The examples showing the necessity of our assumptions and the tightness of our reduction framework are provided in Appendix B and D.
\newline\newline
%\newline
Thank you for your time.
\newline\newline
Sincerely,
\newline
Yiding Feng, Jason D.\ Hartline
and
Yingkai Li

==> Paper/econ-intro.tex <==
This paper shows that some conclusions derived from the simple
economics of optimal auctions \citep{BR-89} approximately extend to
non-linear agents.  For context, optimal mechanisms for non-linear
agents are not simple \citep[e.g.][]{PV-14} and therefore difficult to
understand precisely.  As surveyed by \citep{har-12}, the {\em method
  of approximation} quantifies the extent to which a theory
generalizes from ideal models and separates details from salient
features of the model.

Price posting for single agent with linear utility is optimal
\citep{mye-81, RZ-83}.  This result approximately extends to
single-item multi-agent environments where posting a
while-supplies-last price is approximately optimal.  With a symmetry
assumption (i.e., the agents values are i.i.d.) and regularity
assumption (i.e., the the distribution satisfies a concavity property)
posted pricing is an $e/(e-1)$ approximation \citep{yan-11}; with just
symmetry it is a 2-approximation \citep{CHMS-10}; with just regularity
it is an $e$-approximation \citep{AHNPY-18}.  

The main result of this paper is to quantity the extent to which
agents with non-linear utility resemble agents with linear utility.
For these agents, the approximation bounds above approximately extend.
For a $\beta$-approximation bound for linear agents and non-linear
agents that are $\zeta$-close to resembling linear agents, our result
shows a $\beta\zeta$-approximation bound.  We analyze several
canonical non-linear agent models and give small constant bounds on
how much these non-linear agents resemble linear agents.  For example,
agents with private and independent values and budgets are $\zeta = 3$
close.  This result combines with the results of the previous
paragraph to show that the worst case approximation of posting a price
for such non-linear agents is $3e/(e-1)$ for identical and regular
distributions, $6$ for identical distributions, and $3e$ for regular
distributions.

Our interpretation of these approximation results is as follows.
Though posting a price is not optimal in many environments, the result
that price posting is good is broadly robust.  This result was
previously known for agents with linear utility.  Our results quantify
an aspect of non-linear agents which allows direct comparison to
linear agents with respect to price posting and approximately extends
these robustness results to large and important families of non-linear
agents.  We conclude that, with respect to approximate optimality of
price posting, many kinds of non-linearity of utility are details that
can be omitted from the model without significantly altering the main
take-aways.



==> Paper/extension.tex <==
\section{Conclusions and Extensions}
\label{sec:extension}
In this paper we focused on the approximation bounds for anonymous
pricing in single item environments.  We introduce a generalization of
regularity which characterizes the gap between the price-posting
revenue curve and the ex ante revenue curve.  This generalization
enable a reduction framework to approximately reduce the analysis of
the approximation bound for anonymous pricing for agents with
non-linear utility to that of agents with linear utility.

Generalized regularity property allows other simple versus optimal
results to be lifted from environments with linear utility agents to
ones with non-linear utility agents.  Specifically, simple versus
optimal results that compare some form of posted pricing with an ex
ante relaxation can be directly extended.  For example, \citet{yan-11}
showed that sequential posted pricings, where the agents arrive in a
prescribed order and are offered take-it-or-leave-it
while-supplies-last prices, approximate the ex ante relaxation for
single-item environments, multi-unit environments, and matroid
environments.  The following extension theorem applies where, as
previously in the paper, $\exanterev(\{\revcurve_i\}_{i=1}^n)$ denotes
the ex ante optimal mechanism.
In the literature, 
for linear agents with irregular distributions, 
the randomized sequential posted pricing 
is a constant approximation 
to the optimal revenue. 
Therefore, in our following discussion, 
we show that with randomized prices, 
the results for linear agents 
can be extended to non-linear agents 
with weaker assumptions. 
Finally, we will show that any randomized sequential posted pricing 
can be reduced to sequential posted pricing with weakly higher revenue. 

\begin{definition}
A \emph{sequential per-unit pricing mechanism} is
$(\seq,\seqprices)$ where $\seq$ denotes an ordering of the
agents and $\seqprices$ denotes the price to be offered each agent. 
A \emph{randomized sequential per-unit pricing mechanism} is
$(\seq,\randomseqprices)$ 
where $\randompricei$ is the randomized price for each agent $i$. 
More specifically, 
%for each agent $i$, 
the mechanism first samples per-unit price $\pricei$ 
from $\randompricei$, 
and then posts per-unit price $\pricei$ 
to agent $i$. 
We denote the revenue achieved by the sequential per-unit pricing
mechanism $(\seq,\seqprices)$ for agents with a specific
collection of price-posting revenue curves $\{\cumprice_i\}_{i=1}^n$
by $\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq,\seqprices)$, 
and similarly denote 
$\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq,\randomseqprices)$ 
for the revenue from randomized per-unit pricing mechanism.
\end{definition}


\begin{definition}
Let $\concaveHull$ denote 
the concave hull of the price-posting revenue curve $\cumprice$. 
For any ex ante constraint $\quant$, 
let $\quantTorandomprice(\quant, \concaveHull)$ denote the  
randomized per-unit price such that 
the ex ante probability of 
posting the randomized per-unit 
price $\quantTorandomprice(\quant, \concaveHull)$ 
is $\quant$,  
and the revenue of 
posting the randomized per-unit 
price $\quantTorandomprice(\quant, \concaveHull)$ is $\concaveHull(\quant)$. 
\end{definition}
Intuitively, for any ex ante constraint $\quant$, 
$\concaveHull(\quant)$ is the optimal revenue 
achieved by randomly posting a per-unit price. 
Next we show how to reduce the sequential price-posting mechanism 
for linear agents to 
the sequential price-posting mechanism 
for agents with non-linear utility 
in the downward-closed environment, 
when the concave hull of the price-posting revenue curves 
$\{\concaveHull_i\}_{i=1}^n$ are $\zeta$-close
for ex ante relaxation 
to the ex ante revenue curves $\{\revcurve_i\}_{i=1}^n$.  

\paragraph{Reduction Mechanism} 
For any sequential posted pricing $(\seq,\seqprices)$ for
regular linear utility agents with revenue curves
$\{\revcurve_i\}_{i=1}^n$, 
denote the ex ante constraints corresponding to the sequential prices
$\seqprices$ by $\{\quant_i\}_{i=1}^n$, i.e., $\quant_i =
\priceToQuantile(\price_i, \revcurve_i)$.
Let
$\correspondingquant_i \leq \quant_i$ be the corresponding quantile
for agent $i$ such that 
$\concaveHull_i(\correspondingquant_i) \geq
\frac{1}{\zeta}\revcurve_i(\quant_i)$. 
That is guaranteed to exist by
$\zeta$-closeness for ex ante optimization. 
Let $\availableprob_i$ %= \randomavailableprob_1 = 1$ 
be the probability 
that it is feasible to allocate the item to agent $i$ 
in sequential posted pricing $(\seq,\seqprices)$. 
Consider the sequential
posted pricing mechanism that post 
randomized per-unit price $\randomprice\primed_i$
to each agent $i$ in the same order $\seq\primed = \seq$. 
% Let $\randomprice\primed_1 
% = \quantTorandomprice(\correspondingquant_1, \concaveHull_1)$ 
% be the randomized price posted to the first agent. 
% and let $\randomavailableprob_1 = 1$ 
% be the probability 
% that the first agent receives randomized price 
% $\quantTorandomprice(\quant_1, \concaveHull_1)$. 
For each agent $i$, 
we inductively define the randomized price~$\randomprice\primed_i$, 
and the probability 
that it is feasible to allocate the item to her, 
denoted by~$\feasibleprob_i$. 
Note that $\feasibleprob_i$ only depends on the 
feasibility constraint and the randomized prices 
$\randomprice\primed_1, \dots, \randomprice\primed_{i-1}$, 
not on the randomized price~$\randomprice\primed_i$. 
% and the probability that she receives 
% a finite price when it is feasible to allocate the item to her, 
% denoted by $\randomavailableprob_i$. 
Moreover, we let $\feasibleprob_1 = 1$. 
Then, for each agent $i$, 
let~$\randomprice\primed_i$ be the randomized per-unit price 
%that posts 
$\quantTorandomprice
(\sfrac{(\correspondingquant_i \availableprob_i)}{\feasibleprob_i}, 
\concaveHull_i)$.  
% with probability 
% $\sfrac{\availableprob_i}{\feasibleprob_i}$, 
% and posts price $\infty$ with probability 
% $1 - \sfrac{\availableprob_i}{\feasibleprob_i}$. 
By induction, since the environment is downward-closed, 
for each agent~$i$, $\availableprob_i \leq \feasibleprob_i$, 
and thus the above randomized price is always well defined. 
% Moreover, the probability the each agent $i$ 
% receives finite prices is equivalent, i.e., 
% $\randomavailableprob_i = \availableprob_i$. 


% Let $\availableprob_i, \randomavailableprob_i$ be the probability 
% that it is feasible to allocate the item to agent $i$ 
% in mechanism that sequentially post $\seqprices$ 
% and $\randomseqpricesprimed$ respectively. 

% Let $\randomprice\primed_i$ be the randomized per-unit price 
% that posts randomized per-unit 
% price $\quantTorandomprice(\quant_i, \concaveHull_i)$ 
% with probability 
% $\sfrac{(1-\quant_i)}{(1-\correspondingquant_i)}$, 
% and posts price $0$ with probability 
% $\sfrac{(\quant_i - \correspondingquant_i)}{(1-\correspondingquant_i)}$. 
% Consider the sequential
% posted pricing mechanism that post randomized per-unit price $\randomprice\primed_i$
% to each agent $i$ in the same order $\seq\primed = \seq$. 
% Let $\availableprob_i, \randomavailableprob_i$ be the probability 
% that it is feasible to allocate the item to agent $i$ 
% in mechanism that sequentially post $\seqprices$ 
% and $\randomseqpricesprimed$ respectively. 



\begin{theorem}
\label{t:spp} 
In multi-unit downward-closed environments,
if there is a sequential posted pricing $(\seq,\seqprices)$ for
regular linear utility agents with revenue curves
$\{\revcurve_i\}_{i=1}^n$ that is a $\linearapproxratio$-approximation
to the ex ante relaxation, i.e.,
$\seqpricerev(\{\revcurve_i\}_{i=1}^n,\seq,\seqprices) \geq
\frac{1}{\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$, 
then there is a randomized sequential per-unit
pricing $(\seq\primed,\randomseqpricesprimed)$, 
for non-linear utility agents with
the concave hull of their price-posting revenue curves 
$\{\concaveHull_i\}_{i=1}^n$ that are $\zeta$-close
for ex ante relaxation to their ex ante revenue curves $\{\revcurve_i\}_{i=1}^n$, 
that is a $(\zeta\,\linearapproxratio)$-approximation to the ex ante relaxation, 
i.e., $\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq\primed,\randomseqpricesprimed) \geq
\frac{1}{\zeta\,\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$.
\end{theorem}

\begin{proof} 
Let the randomized sequential per-unit
pricing $(\seq\primed,\randomseqpricesprimed)$ 
be the mechanism defined above. 
% Let $\randomavailableprob_i$ 
% be the probability 
% that agent $i$ receives the randomized posted price 
% $\quantTorandomprice(\correspondingquant_i, \concaveHull_i)$. 
% By our construction, for each agent $i$, 
% the probability that she receives the randomized posted price 
% $\quantTorandomprice(\correspondingquant_i, \concaveHull_i)$ 
% in $(\seq\primed,\randomseqpricesprimed)$
% is equal to the probability she receives the posted price 
% $\pricei$ in $(\seq,\seqprices)$, i.e., 
% $\randomavailableprob_i = \availableprob_i$. 
% Denote the ex ante constraints corresponding to the sequential prices
% $\seqprices$ by $\{\quant_i\}_{i=1}^n$, i.e., $\quant_i =
% \priceToQuantile(\price_i, \revcurve_i)$.  The assumption of the
% theorem implies that sequentially offering the agents the single-agent
% ex ante mechanism corresponding to their ex ante constraint is an
% $\linearapproxratio$-approximation to the ex ante relaxation.  Let
% $\correspondingquant_i \leq \quant_i$ be the corresponding quantile
% for agent $i$ such that 
% $\concaveHull_i(\correspondingquant_i) \geq
% \frac{1}{\zeta}\revcurve_i(\quant_i)$. 
% That is guaranteed to exist by
% $\zeta$-closeness for ex ante optimization. 
% Let $\randomprice\primed_i$ be the randomized per-unit price 
% that posts randomized per-unit 
% price $\quantTorandomprice(\quant_i, \concaveHull_i)$ 
% with probability 
% $\sfrac{(1-\quant_i)}{(1-\correspondingquant_i)}$, 
% and posts price $0$ with probability 
% $\sfrac{(\quant_i - \correspondingquant_i)}{(1-\correspondingquant_i)}$. 
% Consider the sequential
% posted pricing mechanism that post randomized per-unit price $\randomprice\primed_i$
% %$\price\primed_i =
% %\cumprice_i(\correspondingquant_i)/
% %\correspondingquant_i$
% to each agent $i$ in the same order $\seq\primed = \seq$. 
% Let $\availableprob_i, \randomavailableprob_i$ be the probability 
% that it is feasible to allocate the item to agent $i$ 
% in mechanism that sequentially post $\seqprices$ 
% and $\randomseqpricesprimed$ respectively. 
% Note that in mechanism that 
% sequentially post $\randomseqpricesprimed$, 
% the probability that any agent $i$ 
% will accept the randomized per-unit 
% price $\randomprice\primed_i$ is $\quant_i$. 
% Since the order of the agents are the same, 
% for any agent $i$, 
% the probability that it is feasible to allocate the 
% item to her is equivalent under two mechanisms, i.e., 
% $\availableprob_i = \randomavailableprob_i$.
% The probability that the item is available 
% when agent $i$ comes is 
% $\textstyle{\prod_{1\leq j < i}
% (1 - \quant_j)}$
% and 
% $\textstyle{\prod_{1\leq j < i}
% (1 - \correspondingquant_j)}$
% respectively in these two mechanisms.
For each agent $i$, 
the probability 
that it is feasible to allocate the item to her 
in $(\seq\primed,\randomseqpricesprimed)$
and in $(\seq,\seqprices)$ 
are 
$\feasibleprob_i$ and $\availableprob$, respectively. 
Condition on the event that 
it is feasible to allocate the item to agent~$i$, 
% receives the randomized posted price 
% $\quantTorandomprice(\correspondingquant_i, \concaveHull_i)$
% and the posted price $\pricei$,
the expected revenue from her is 
$\concaveHull(\sfrac{(\correspondingquant_i \availableprob_i)}{\feasibleprob_i})$ 
and $\revcurve(\quant_i)$, respectively. 
Since $\concaveHull$ is concave, we have 
$\concaveHull(\sfrac{(\correspondingquant_i \availableprob_i)}{\feasibleprob_i})
\geq \sfrac{ \availableprob_i }{\feasibleprob_i} 
\concaveHull(\correspondingquant_i)$.
Thus, %NEEDS CORRECTION FOR GENERAL ENVIRONMENTS.
\begin{align*}
\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq\primed,\randomseqpricesprimed)
    &= \sum_{i=1}^n 
    %\left(\prod_{1\leq j < i} 
    %(1-\correspondingquant_j) \right)
    \feasibleprob_i \cdot 
    \concaveHull_i
    \left(\frac{\correspondingquant_i \availableprob_i}{\feasibleprob_i} \right)  
    \geq \frac{1}{\zeta} \sum_{i=1}^n 
    %\left(\prod_{1\leq j < i} (1-\quant_j)\right)
    \availableprob_i \cdot
    \revcurve_i(\quant_i) 
    \geq \frac{1}{\zeta\,\linearapproxratio} \cdot \exanterev(\{\revcurve_i\}_{i=1}^n). \qedhere
\end{align*}
\end{proof}


The mechanism in \Cref{t:spp} can be derandomized. 
The idea is that for any randomized prices, 
there exists a deterministic price in the support of the 
randomized prices such that 
the expected revenue of posting the deterministic price 
is weakly higher. 
% The idea is that since the randomized price is a 
% $\zeta\,\linearapproxratio$-approximation to the ex ante relaxation, 
% there exists a deterministic price in the support of the 
% randomized prices such that 
% the expected revenue of posting the deterministic price 
% is also a $\zeta\,\linearapproxratio$-approximation 
% to the ex ante relaxation. 
Moreover, we can find a weakly better deterministic posted pricing mechanism 
% that is weakly better 
% than the randomized mechanism defined in \Cref{t:spp} 
by 
choosing the optimal deterministic price inductively for each agent. 
Note that the best price for each agent can be efficiently approximated 
through Monte Carlo sampling. 

\begin{lemma}
For any randomized sequential per-unit
pricing $(\seq, \randomseqprices)$ 
for agents with price-posting revenue curve $\{\cumprice_i\}_{i=1}^n$, 
there exists a sequential per-unit
pricing $(\seq, \seqprices)$ with weakly higher expected revenue, 
i.e., $\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq,\seqprices) \geq
\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq,\randomseqprices)$.
\end{lemma}

% \begin{corollary}
% In multi-unit  with general feasibility constraint, %downward closed environments,
% if there is a sequential posted pricing $(\seq,\seqprices)$ for
% regular linear utility agents with revenue curves
% $\{\revcurve_i\}_{i=1}^n$ that is a $\linearapproxratio$-approximation
% to the ex ante relaxation, i.e.,
% $\seqpricerev(\{\revcurve_i\}_{i=1}^n,\seq,\seqprices) \geq
% \frac{1}{\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$, 
% then there is a sequential per-unit
% pricing $(\seq\primed,\seqpricesprimed)$ 
% that is a $\zeta\,\linearapproxratio$-approximation to the ex ante relaxation 
% for non-linear utility agents with
% the concave hull of their price-posting revenue curves 
% $\{\concaveHull_i\}_{i=1}^n$ that are $\zeta$-close
% for ex ante relaxation to their ex ante revenue curves $\{\revcurve_i\}_{i=1}^n$, 
% i.e., $\seqpricerev(\{\cumprice_i\}_{i=1}^n,\seq\primed,\seqpricesprimed) \geq
% \frac{1}{\zeta\,\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$.
% \end{corollary}

\Cref{t:spp} is similar to an extension theorem discussed in
\citet{AFHH-13} which shows that, under the same assumptions,
sequentially running the single-agent ex ante optimal mechanisms
is a $\linearapproxratio$-approximation to the ex ante relaxation
(assumption the $\linearapproxratio$-approximation ratio holds for
regular linear utility agents with the same revenue curves).  The
advantage of our results over those of \citet{AFHH-13} is that
single-agent posted pricings are simpler and easier to compute than
the single-agent ex ante optimal mechanisms.  The advantage of
\citet{AFHH-13} is that it does not require any version of regularity.

For single-item, matroid, and $k$-unit (unit-demand) environments with
regular linear utility agents, \citet{yan-11} shows that sequential
posted pricing are $\sfrac{e}{(e-1)}$, $\sfrac{e}{(e-1)}$, and $(1-\sfrac 1
{\sqrt{2\pi k}})^{-1}$ approximations, respectively.  For example, \Cref{t:spp} and
combines with \Cref{thm:public 2e bound} for regular public budget
agents show that public budget agents with regular decreasing-density
valuation distributions admit the same approximation bounds in the
three environments mentioned above.
 


==> Paper/new_result/framework.tex <==
\section{Reduction Framework}
When the agent's price-posting revenue curve is concave, 
we have a different approach for analyzing 
the approximation ratio of the anonymous pricing mechanism. 

\begin{definition}
The agent's price-posting revenue curve $\cumprice$ 
is downward $(\alpha, \beta)$-close 
to her ex ante revenue curve $\revcurve$, if 
for all $\quant \in [0, 1/\beta]$, 
there exists a quantile 
$\correspondingquant \leq \quant$ such that 
$\cumprice(\correspondingquant) \geq \frac{1}{\alpha} \revcurve(\quant)$. 
\end{definition}

Note that the agent's price-posting revenue curve $\cumprice$ 
is $(\alpha, \beta)$-close 
to her ex ante revenue curve $\revcurve$
implies that 
her price-posting revenue curve $\cumprice$ 
is downward $(\alpha, \beta)$-close 
to her ex ante revenue curve $\revcurve$. 

\begin{theorem}
%\label{thm:general EAR bound}
Given agents with 
ex ante revenue 
curves 
$\{\revcurve_i\}_{i=1}^n$
and price-posting revenue curves
$\{\cumprice_i\}_{i=1}^n$,
if for each agent $i$, 
her price-posting revenue curve $\cumprice_i$
is downward $(\alpha, \beta)$-close 
to her ex ante revenue curve $\revcurve_i$, 
then
the optimal ex ante relaxation on revenue curves 
$\{\cumprice_i\}_{i=1}^n$ 
is an $(\alpha\beta)$-approximation
to the optimal ex ante relaxation on revenue curves 
$\{\revcurve_i\}_{i=1}^n$,  
i.e.,
$\exanterev(\{\cumprice_i\}_{i=1}^n)
\geq \frac{1}{\alpha \beta}
\exanterev(\{\revcurve_i\}_{i=1}^n)$. 
\end{theorem}
\begin{proof}
Let $\quant_i$ be the optimal ex ante relaxation for 
ex ante revenue curves 
$\{\revcurve_i\}_{i=1}^n$, 
and let $\quant'_i = \min\{\quant_i, \frac{1}{\beta}\}$. 
%By \Cref{lem:ex-ante is concave}, the ex ante revenue curve is concave. 
We know that $\revcurve_i(\quant'_i) 
\geq \frac{1}{\beta} \revcurve_i (\quant_i)$. 
Moreover, let $\correspondingquant_i$ be the corresponding quantile 
such that 
$\correspondingquant_i \leq \quant'_i$ 
and $\cumprice_i(\correspondingquant_i) 
\geq \frac{1}{\alpha}\revcurve(\quant'_i)$, 
we have 
\begin{equation*}
    \exanterev(\{\cumprice_i\}_{i=1}^n) 
    \geq \sum_i \cumprice_i(\correspondingquant_i) 
    \geq \frac{1}{\alpha \beta} \sum_i \revcurve(\quant_i) 
    = \frac{1}{\alpha \beta} \exanterev(\{\revcurve_i\}_{i=1}^n). \qedhere
\end{equation*}
\end{proof}

\begin{corollary}
%For the single item environment, 
If for each agent $i$, 
her price-posting revenue curve $\cumprice_i$
is concave, 
and is downward $(\alpha, \beta)$-close 
to her ex ante revenue curve $\revcurve_i$, 
then 
the worst case approximation factor of 
anonymous pricing to the ex ante relaxation 
is
$\alpha \beta \rho$.
\end{corollary}

\begin{figure}[t]
\centering
\input{Paper/new_result/figure-reduction.tex}
\caption{\label{f:framework} 
The reduction framework.
}
\end{figure}

==> Paper/new_result/improved-framework-Beta.tex <==
\section{Improved Framework for $\ln \beta$}

% In this section, we first consider the simple case 
% when each agent has linear utility 
% and the value distribution is irregular. 
% Moreover, we require that 
% the price-posting revenue curve $\cumprice_i$ 
% $(1, \beta)$-close for price posting
% to the ex ante revenue curve $\revcurve_i$. 

% Let $\{\optquant_i\}_{i=1}^n$ be the quantile 
% that maximize the optimal ex ante revenue 
% subject to the constraint that 
% $\sum_i \optquant_i \leq 1$. 
% Therefore, there exists at most 1 agent such that 
% $\optquant_i > \sfrac{1}{2}$. 
% Moreover, there exists at most $\beta$ agent 
% such that 
% $\optquant_i > \sfrac{1}{\beta}$. 

% We partition the agents into three groups 
% according to their optimal ex ante probability $\optquant_i$. 
% Let $\group_1 = \{i : \optquant_i \leq \sfrac{1}{\beta}\}$, 
% $\group_2 = \{i : \sfrac{1}{\beta} < \optquant_i \leq \sfrac{1}{2}\}$, 
% and $\group_3 = \{i : \optquant_i > \sfrac{1}{2}\}$.
% Let $k$ be the group with maximum ex ante revenue. 
% If $k = 1$, 
% \begin{equation*}
% \pricerev(\{\cumprice_i\}_{i=1}^n) 
% \geq \pricerev(\{\cumprice_i\}_{i\in \group_1})
% \geq \frac{1}{\linearapproxratio} 
% \exanterev(\{\revcurve_i\}_{i\in \group_1}) 
% \geq \frac{1}{3\linearapproxratio} 
% \exanterev(\{\revcurve_i\}_{i=1}^n). 
% \end{equation*}




\begin{lemma}
\label{lem:ln beta approx between rev and welfare}
For a single agent with value distribution supported in $[a, b]$, 
the maximum ratio between the welfare and price posting 
is $\ln \sfrac{b}{a}$. 
\end{lemma}


\begin{theorem}\label{thm:improved AP ln bound}
Given agents with 
ex ante revenue curves 
$\{\revcurve_i\}_{i=1}^n$
and price-posting revenue curves
$\{\cumprice_i\}_{i=1}^n$,
if the revenue of posting effective price $\exanteprice$ 
on revenue curve $\{\revcurve_i\}_{i=1}^n$
is a 
$\linearapproxratio$-approximation to the ex ante relaxation
revenue of those agents, 
i.e., 
$\pricerev(
\{\revcurve_i\}_{i=1}^n, \exanteprice) 
\geq \frac{1}{\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$, 
for any agent $i$, 
the price-posting revenue curve $\cumprice_i$ 
$(\alpha, \beta)$-close for price posting
to the ex ante 
revenue curve $\revcurve_i$, 
and the 
optimal price posting revenue 
for each agent $i$
is an $\eta$-approximation to the  
optimal single agent revenue, 
then
posting anonymous price 
is a $(\improvedAPln)$-approximation
to the ex ante relaxation, 
i.e.,
$
(\improvedAPln)
\cdot \pricerev(\{\cumprice_i\}_{i=1}^n) 
\geq 
\exanterev(\{\revcurve_i\}_{i=1}^n)$. 
\end{theorem}

\begin{proof}[Proof of \Cref{thm:improved AP ln bound}]
We consider the following two different cases
whether there is an agent with 
significant contribution of 
revenue in 
$\pricerev(\{\revcurve_i\}_{i=1}^n, \exanteprice)$.
Specifically, agent $i$
is a significant contributor 
if $\priceToQuantile(\exanteprice, \revcurve_i)$
is at least $\sfrac{1}{2}$.
\paragraph{When Significant Contributor Exists}
Suppose there exists an agent $i^*$ such that 
$\priceToQuantile(\exanteprice, \revcurve_{i^*})$
is at least $\sfrac{1}{2}$.
Consider the optimal price-posting 
for this single agent $i^*$.
Its revenue is 
a $2 \eta \linearapproxratio$-approximation 
to the ex ante relaxation, i.e., 
\begin{align*}
\max_{\quant} \cumprice_{i^*}(\quant) 
\geq \frac{1}{\eta} \max_{\quant}
\revcurve_{i^*}(\quant) 
\geq \frac{1}{2 \eta}
\pricerev(
\{\revcurve_i\}_{i=1}^n, \exanteprice) 
\geq \frac{1}{2 \eta \gamma} 
\exanterev(\{\revcurve_i\}_{i=1}^n)
\end{align*} 
where the first inequality is 
due to our $\eta$-approximation assumption
for a single agent,
and the second inequality 
is 
due to the fact 
that agent $i^*$ is a significant contributor.

\paragraph{When Significant Contributor Does Not Exist}
Suppose there is no significant contributor,
i.e.,
$\priceToQuantile(\exanteprice, \revcurve_{i}) 
< \sfrac{1}{2}$ for all $i$. 
Next we partition the agents into 2 different groups. 
Let $\group_1 = \{i : 
\priceToQuantile(\exanteprice, \revcurve_{i}) 
\leq \sfrac{1}{\beta}\}$, 
and 
$\group_2 = \{i : \sfrac{1}{\beta} < 
\priceToQuantile(\exanteprice, \revcurve_{i}) 
\leq \sfrac{1}{2}\}$. 
If 
$\pricerev(\{\revcurve_i\}_{i\in \group_1}, \exanteprice)
\geq \pricerev(\{\revcurve_i\}_{i\in \group_2}, \exanteprice)$, 
we have 
\begin{eqnarray*}
    \pricerev\left(\{\cumprice_i\}_{i\in \group_1},
    \frac{\exanteprice}{\alpha}\right) 
    &=& \frac{\exanteprice}{\alpha} \cdot 
    \left(1 - \prod\nolimits_{i\in \group_1} (1-\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i)) \right) \\
    &\geq& \frac{\exanteprice}{\alpha} 
    \cdot \left(1 - \prod\nolimits_{i\in \group_1} 
    (1 - \priceToQuantile(\exanteprice, \revcurve_i)) \right) 
    = \frac{1}{\alpha}
    \pricerev(\{\revcurve_i\}_{i\in \group_1}, \exanteprice) \\
    &\geq&\frac{1}{2 \alpha } \pricerev(\{\revcurve_i\}_{i=1}^n, \exanteprice) 
    \geq \frac{1}{2 \alpha \linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n). 
\end{eqnarray*}

Next we consider the case when  
$\pricerev(\{\revcurve_i\}_{i\in \group_1}, \exanteprice)
< \pricerev(\{\revcurve_i\}_{i\in \group_2}, \exanteprice)$. 
If $\abs{\group_2} \geq \beta$,
% let $\group_3 \subseteq \group_2$ 
% such that $\abs{\group_3} = \beta$,
% and 
we have, 
\begin{eqnarray*}
\pricerev\left(\{\cumprice_i\}_{i\in \group_2},
\frac{\exanteprice}{\alpha} \right) 
&=& \frac{\exanteprice}{\alpha} \cdot 
\left(1 - \prod\nolimits_{i\in \group_2} 
(1-\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i)) \right) \\
&\geq& \frac{\exanteprice}{\alpha} 
\cdot \left(1 - \prod\nolimits_{i\in \group_2} 
(1 - \frac{1}{\beta}) \right) 
\geq \frac{e \exanteprice}{(e-1) \alpha} \\
&\geq& \frac{e}{(e-1) \alpha} \pricerev(\{\revcurve_i\}_{i=1}^n, \exanteprice)
\geq \frac{e}{(e-1) \alpha \linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n). 
\end{eqnarray*}


{\color{red}
Currently assume that $\concaveHull$ 
is $\eta$-close for ex ante optimization
to ex ante revenue curve $\revcurve_i$. 
}

In the case $\abs{\group_2} < \beta$, 
note that the equivalent price 
for ex ante revenue curve $\revcurve_i$
that corresponds to 
quantile $\frac{1}{\beta}$ 
is at most $2 \exanteprice \beta$. 
Since the distribution above $2 \exanteprice \beta$
does not affect the revenue of anonymous pricing 
of $\exanteprice$ for agents in $\group_2$, 
we construct the truncated price posting revenue curve 
$\{\truncateCumprice_i\}_{i\in \group_2}$, 
and the truncated ex ante revenue curve 
$\{\truncateExante_i\}_{i\in \group_2}$. 
Let $\truncateHull_i$ be the concave hull for 
$\truncateCumprice_i$. 
We know that $\truncateHull_i$ 
is $\max\{\alpha, \eta\}$-close for ex ante optimization
to ex ante revenue curve $\truncateExante_i$. 
Therefore, 
\begin{eqnarray*}
\max\{\alpha, \eta\} \cdot  \pricerev(\{\truncateHull_i\}_{i\in \group_2})
\geq \pricerev(\{\truncateExante_i\}_{i\in \group_2})
\geq \pricerev(\{\revcurve_i\}_{i\in \group_2}, \exanteprice)
\end{eqnarray*}
By \Cref{lem:ln beta approx between rev and welfare},
\begin{eqnarray*}
(1 + 3\ln \beta)\pricerev(\{\truncateCumprice_i\}_{i\in \group_2})
\geq
\welfare(\{\truncateHull_i\}_{i\in \group_2})
\geq
\pricerev(\{\truncateHull_i\}_{i\in \group_2})
\end{eqnarray*}
Thus, 
\begin{eqnarray*}
\pricerev(\{\cumprice_i\}_{i\in \group_2})
&\geq&
\frac{1}{(1 + 3\ln \beta)\max\{\alpha, \eta\}}
\pricerev(\{\truncateHull_i\}_{i\in \group_2}) \\
&\geq& 
\frac{1}{2e(1 + 3\ln \beta)\max\{\alpha, \eta\}}
\exanterev(\{\revcurve_i\}_{i=1}^n). 
\end{eqnarray*}

\end{proof}


==> Paper/new_result/improved-framework.tex <==
\section{Improved Framework}
\label{sec:improved framework}

Here we give an analogy results as in 
\Cref{thm:general AP bound} with 
an additional parameter for
the approximation ratio of 
the single-agent pricing (denoted as $\eta$ in 
the theorem)
and 
a more careful 
analysis. 
\Cref{thm:general AP bound} is an immediate 
corollary from it and the approximation 
bound for private-budget section can be improved 
from $O(\kappa^2)$ to $O(\kappa)$.

\begin{theorem}\label{thm:improved AP bound}
Given agents with 
ex ante revenue 
curves 
$\{\revcurve_i\}_{i=1}^n$
and price-posting revenue curves
$\{\cumprice_i\}_{i=1}^n$,
if the revenue of posting effective price $\exanteprice$ 
on revenue curve $\{\revcurve_i\}_{i=1}^n$
is a 
$\linearapproxratio$-approximation to the ex ante relaxation
revenue of those agents, 
i.e., 
$\pricerev(
\{\revcurve_i\}_{i=1}^n, \exanteprice) 
\geq \frac{1}{\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$, 
for any agent $i$, 
the price-posting revenue curve $\cumprice_i$ 
$(\alpha, \beta)$-close for price posting
to the ex ante 
revenue curve $\revcurve_i$, 
and 
the 
optimal price posting revenue 
for each agent $i$
is an $\eta$-approximation to the  
optimal single agent revenue, 
then
posting anonymous price 
%$\sfrac{\exanteprice}{\alpha}$
is a $(\improvedAP)$-approximation
to the ex ante relaxation, 
i.e.,
$
(\improvedAP)
\cdot \pricerev(\{\cumprice_i\}_{i=1}^n)%, 
%\frac{\exanteprice}{\alpha})
\geq 
%\frac{1}{\max\{\alpha, \sqrt{\alpha\beta}\} 
%\eta \gamma}
\exanterev(\{\revcurve_i\}_{i=1}^n)$. 
\end{theorem}

Notice that 
comparing to \Cref{thm:general AP bound},
the $\eta$-approximation for single-agent pricing 
is the only additional assumption stated
in 
\Cref{thm:improved AP bound}, and 
$(\alpha, \beta)$-regular 
implies that 
% the optimal price-posting 
% revenue for this single agent 
% is at least an $\sfrac{1}{\alpha \beta}$
% fraction of the optimal revenue 
% for this agent,
% i.e.,
the parameter $\eta$ is at most 
$\alpha\beta$.

\begin{proof}[Proof of \Cref{thm:improved AP bound}]
We consider the following two different cases
whether there is an agent with 
significant contribution of 
revenue in 
$\pricerev(\{\revcurve_i\}_{i=1}^n, \exanteprice)$.
Specifically, agent $i$
is a significant contributor 
if $\priceToQuantile(\exanteprice, \revcurve_i)$
is at least $\sfrac{1}{\threshold}$,
where $\threshold$ is a threshold tuned at 
the end of our proof.
\paragraph{When Significant Contributor Exists}
Suppose there exists an agent $i^*$ such that 
$\priceToQuantile(\exanteprice, \revcurve_{i^*})$
is at least $\sfrac{1}{\threshold}$.
Consider the optimal price-posting 
for this single agent $i^*$.
Its revenue is 
a $\threshold \eta \linearapproxratio$-approximation 
to the ex ante relaxation, i.e., 
\begin{align*}
\max_{\quant} \cumprice_{i^*}(\quant) 
\geq \frac{1}{\eta} \max_{\quant}
\revcurve_{i^*}(\quant) 
\geq \frac{1}{\eta \threshold}
\pricerev(
\{\revcurve_i\}_{i=1}^n, \exanteprice) 
\geq \frac{1}{\eta \threshold \gamma} 
\exanterev(\{\revcurve_i\}_{i=1}^n)
\end{align*} 
where the first inequality is 
due to our $\eta$-approximation assumption
for a single agent,
and the second inequality 
is 
due to the fact 
that agent $i^*$ is a significant contributor.
\paragraph{When Significant Contributor Does Not Exist}
Suppose there is no significant contributor,
i.e.,
$\priceToQuantile(\exanteprice, \revcurve_{i}) 
< \sfrac{1}{\threshold}$ for all $i$.
Under a similar argument in
\Cref{lem:close rev curve imply close pricing}, 
we can lower bound 
$\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i)$
for every agent $i$ as follows,
\begin{align*}
    \priceToQuantile
    \left(\frac{\exanteprice}{\alpha}, \cumprice_i
    \right)
    \geq 
    \left\{
    \begin{array}{ll}
      \priceToQuantile(\exanteprice, \revcurve_i)
      &
      \text{ if }
      \priceToQuantile(\exanteprice, \revcurve_{i}) 
\leq \sfrac{1}{\beta}\\
      \frac{\threshold}{\beta} \cdot 
\priceToQuantile(\exanteprice, \revcurve_i)
     & \text{ otherwise}
    \end{array}
    \right.
\end{align*}
where we use the fact that 
$\priceToQuantile
\left(\frac{\exanteprice}{\alpha}, \cumprice_i \right)
\geq \sfrac{1}{\beta}$ 
and 
$\priceToQuantile(\exanteprice, \revcurve_{i}) 
< \sfrac{1}{\threshold}$
    in the latter case. 
%for any price $\exanteprice$ with quantile 
%$\quant(\exanteprice) \leq \frac{1}{\threshold}$, 
% if $\priceToQuantile(\exanteprice, \revcurve_{i}) 
% \leq \sfrac{1}{\beta}$, 
% $\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i) 
% \geq \priceToQuantile(\exanteprice, \revcurve_i)$;
% otherwise
% (if $
% \priceToQuantile(\exanteprice, \revcurve_{i})  > \sfrac{1}{\beta}$), 
% $\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i) 
% \geq \frac{1}{\beta} 
% \geq \frac{\threshold}{\beta} \cdot 
% \priceToQuantile(\exanteprice, \revcurve)$. 
Therefore, for parameter $\threshold \leq \beta$, 
% if for all agents $i$, 
% the quantile of agent $i$ for posting price
% $\exanteprice$ is at most $\sfrac{1}{\threshold}$, 
the the revenue of posting price $\frac{\exanteprice}{\alpha}$ 
% in the original instance 
is 
\begin{eqnarray*}
    \pricerev\left(\{\cumprice_i\}_{i=1}^n,
    \frac{\exanteprice}{\alpha}\right) 
    &=& \frac{\exanteprice}{\alpha} \cdot 
    \left(1 - \prod\nolimits_i (1-\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i)) \right) 
    \geq \frac{\exanteprice}{\alpha} \cdot 
    \left(1 - \prod\nolimits_i (1 - \frac{\threshold}{\beta}
    \priceToQuantile(\exanteprice, \revcurve_i)) \right) \\
    &\geq& \frac{\exanteprice \threshold}{\alpha\beta} 
    \cdot \left(1 - \prod\nolimits_i 
    (1 - \priceToQuantile(\exanteprice, \revcurve_i)) \right) 
    = \frac{\threshold}{\alpha\beta}
    \pricerev(\{\revcurve_i\}_{i=1}^n, \exanteprice) \\
    &\geq&\frac{\threshold}{\alpha \beta \linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n). 
\end{eqnarray*}

To balance the approximation ratio
for both cases,
%if $\sqrt{\sfrac{\alpha \beta}{\eta}} \leq \beta$, 
if $\alpha \leq \beta \eta$, 
setting 
$\threshold = \sqrt{\sfrac{\alpha \beta}{\eta}}$
optimizes the approximation ratio as 
$\sqrt{\alpha \beta \eta} \cdot \linearapproxratio$;
and 
%if $\sqrt{\sfrac{\alpha \beta}{\eta}} > \beta$,  
if $\alpha > \beta \eta$,
setting $\threshold = \beta$
optimizes
the approximation ratio as $\alpha \linearapproxratio$. 
% Note that this result is an improvement 
% comparing to \ref{thm:general AP bound} 
% since $\eta \leq \alpha \beta$ 
% by the concavity of the ex ante revenue curve. 
\end{proof}

==> Paper/new_result/mhr-improved.tex <==
 \section{MHR Budget Distribution}

Assuming that
the value and the budget 
are independently distributed,
the valuation distribution is regular,
and
the budget distribution 
is MHR, 
the price-posting revenue curve is concave. 
This result is formally stated in \Cref{lem:private budget concave price-posting revenue curve}, 
whose proof is deferred to 
Appendix~\ref{apx:private}. 
Due to the concavity of the price-posting revenue curve, 
we show
a better approximation bound 
for anonymous pricing 
using the reduction in \Cref{thm:general EAR bound}. 
% by
% \Cref{thm:general EAR bound}.
% The proof of \Cref{lem:private budget concave price-posting revenue curve}
% %and \Cref{thm: private budget MHR}
% is deferred to 
% Appendix~\ref{apx:private}.


\begin{lemma}\label{lem:private budget concavity}
A single
agent with 
private-budget utility 
has a concave price-posting 
revenue curve $\cumprice$ 
if 
her value and budget 
are independently distributed,
the valuation distribution is regular,
and the budget distribution is MHR.
%under \Cref{asp:value budget independent},
%\ref{asp:value regular},
%\ref{asp:budget MHR},
\end{lemma}

% With \Cref{lem:private budget concave price-posting revenue curve}, 
% the price-posting revenue is concave, 
% and we are able to achieve better bounds for 
% MHR budget distributions by applying the approach 
% in \Cref{cor:ex ante close}. 


\begin{theorem}\label{thm: private budget MHR improved}
A single agent 
with private-budget utility 
has a price-posting revenue curve $\cumprice$ 
that is $\mhrbound$-close for ex ante optimization 
to her ex ante revenue curve $\revcurve$, 
if 
her value and budget 
are independently
distributed,
the valuation distribution is regular,
and the budget distribution is MHR. 
\end{theorem}

\begin{corollary}
For a single item 
environment with 
agents with private-budget utility,
the worst case
approximation factor of
anonymous pricing to the ex ante
relaxation is at most $\mhrbound\rho$
if values and budgets 
are independently distributed,
the valuation distributions are regular,
and the budget distributions are MHR.
\end{corollary}

The high level idea is similar
as the previous subsection.
Fix any ex ante constraint $\quant$,
we decompose the ex ante mechanism 
$\EX$ 
into $\EXS$ and $\EXL$
where 
the per-unit prices in $\EXS$
for all types are at most 
the market 
clearing price
and the per-unit prices in $\EXL$
for all types are larger than 
the market 
clearing price.
\Cref{lem:EXS} upper bounds the revenue of $\EXS$
and
\Cref{lem:market clearing price large},
\Cref{lem:market clearing price small}
and upper bound the revenue of
$\EXL$.
Specifically, when the market clearing price is large
than the Myerson reserve,
\Cref{lem:EXS} and
\Cref{lem:market clearing price large}
guarantees that posting the market clearing 
price is a 2-approximation 
to $\EX$.
In this subsection, 
we improve the remaining case
where the market clearing price is smaller 
than the Myerson reserve.
This improvement is due to
the fact that
closeness for ex ante optimization 
allows us to consider 
posting any price
at least the market clearing price,
i.e., the ex ante constraint 
does not need to bind.
See Figure \Cref{XS}.
Specifically, 
we will use a similar technique 
in \Cref{lem:single agent approx public}
which considers a random price drawn 
from valuation distribution. 
The main difference is that
if the realization of the random price
is smaller than the the market clearing price,
to satisfies the ex ante constraint,
we replace it with the market clearing price.


\begin{lemma}
\label{lem:posting randomized price for EXL}
For a single agent 
with private-budget utility,
independently distributed value 
and budget,
a regular distribution, 
if the market clearing price 
$\price = \sfrac{\cumprice(\quant)}{\quant}$ 
is smaller than the Myerson's reserve, 
there exists $\quant\primed \leq \quant$
such that 
the market clearing revenue from $\quant\primed$
is a 2-approximation 
to the revenue from $\EXL$, 
i.e., 
$2 \cumprice(\quant\primed) \geq 
%\int_{\lbudget}^{\hbudget} \Rev[\wealth]{\EXL} dG(\wealth)
\Rev{\EXL}
$.
\end{lemma}

\begin{proof}
Let $\OPT_\wealth$ be the optimal mechanism
to types with budget $\wealth$
without ex ante constraint
and 
$\Rev[\wealth]{\OPT_\wealth}$ be its expected 
revenue 
from these types.
Let
$\Rev[\wealth]{\price}$
be the expected 
revenue 
from posting price $\price$
to types with budget $\wealth$.
We consider
the revenue from types
with every fixed budget level separately. 
For types with budget smaller than
the market clearing price $\price$, 
i.e., $\wealth < \price$, 
budget binds for those types under market clearing price. 
Therefore, 
the revenue from those types in 
$\EXL$ 
is upper bounded by the revenue from those types 
in
posting the market clearing price $\price$,
i.e., $\Rev[\wealth]{\EXL} \leq \Rev[\wealth]{\price}$.
For types with budget larger than the market clearing price, 
i.e., $\wealth \geq \price$, 
the revenue from types with budget $\wealth$ is 
upper bounded by 
the optimal revenue for budget $\wealth$,
i.e., $\Rev[\wealth]{\EXL} \leq \Rev[\wealth]{\OPT_\wealth}$.
Therefore, 
The revenue for $\EXL$ is upper bounded by 
\begin{align*}
\Rev{\EXL} &= 
\int_{\lbudget}^{\price} \Rev[\wealth]{\EXL} dG(\wealth)
+ \int_{\price}^{\hbudget} \Rev[\wealth]{\EXL} dG(\wealth) \\
& \leq \int_{\lbudget}^{\price} \Rev[\wealth]{\price} dG(\wealth)
+ \int_{\price}^{\hbudget} \Rev[\wealth]{\OPT} dG(\wealth).
\end{align*}

Consider the mechanism that draws a random price 
$\randomprice_0$
from the valuation distribution $F$
and post a per-unit price 
$\randomprice$ equal to the maximum
between the market clearing price $\price$
and this random price $\randomprice_0$,
i.e., $\randomprice = 
\max\{\price, \randomprice_0\}$.
In the argument below, we use 
$\randomprice$ to denote this random price 
and its realization.
Clearly, this mechanism satisfies 
the ex ante constraint $\quant$ since 
$\randomprice \geq \price$ and $\price$ is 
the market clearing price under $\quant$.
Let 
$\randomquant = 1 - F(\randomprice)$
be the probability that the value $\val$
is at least $\randomprice$.
Note that $\randomquant$
is a random variable fully depends on
$\randomprice$.
For any fixed $\wealth$, 
when $\randomprice \in [\price, \wealth]$, 
the revenue of posting price $\randomprice$ 
is $\cumpricelinear(\randomquant)$
where $\cumpricelinear$
is the price-posting revenue curve without budget;
and when $\randomprice > \wealth$, 
the revenue of posting price $\randomprice$ 
is $\wealth \randomquant$. 

Next, we use $\Rev[\wealth]{\randomprice}$
to upper bound 
$\Rev[\wealth]{\price}$ for all $\wealth < \price$
and 
$\Rev[\wealth]{\OPT_\wealth}$ for all $\wealth \geq \price$.
The following argument has a 
clear geometric interpretation
which is also illustrated
in \Cref{f:revenue of sample}.


For types with fixed 
$\wealth < \price$,
the revenue of posting the market clearing 
price $\price$, 
i.e., $\Rev[\wealth]{\price}$ is
$
(1 - F(\price))\wealth$.
On the other hand,
the revenue of posting the random 
price $\randomprice$
is 
$$\Rev[\wealth]{\randomprice} =
\Rev[\wealth]{\randomprice 
| \randomprice > \price}
+
\Rev[\wealth]{\randomprice 
| \randomprice = \price}
=
\int_0^{1-F(\price)}
\wealth\quant\, d\quant
+
\wealth(1-F(\price))F(\price).
$$
Hence, $\Rev[\wealth]{\price}
\leq 2\Rev[\wealth]{\randomprice}$
for all $\wealth < \price$.


For types with fixed 
$\wealth \geq \price$,
\Cref{lem:public budget optimal under regular}
implies that 
$\OPT_\wealth$
is
posting 
the minimum between
budget $\wealth$
and Myerson reserve $\myersonReserve$.
Since we assume 
that $\myersonReserve$
is larger than the market clearing price,
$\Rev[\wealth]{\OPT_\wealth} = 
\max_{ 1-F(\wealth)\leq\quant \leq 1-F(\price)}
\cumpricelinear(\quant)$.
On the other hand,
the revenue of posting the random 
price $\randomprice$
is 
\begin{align*}
\Rev[\wealth]{\randomprice} &=
\Rev[\wealth]{\randomprice 
| \randomprice > \wealth}
+
\Rev[\wealth]{\randomprice 
| \wealth\geq \randomprice > \price}
+
\Rev[\wealth]{\randomprice 
| \randomprice = \price} \\
&=
\int_0^{1-F(\wealth)}
\wealth\quant\, d\quant
+
\int_{1-F(\wealth)}^{1-F(\price)}
\cumpricelinear(\quant)\, d\quant
+
\wealth(1-F(\price))F(\price).
\end{align*}
Since valuation is regular,
i.e., 
$\cumpricelinear$ is concave,
$\Rev[\wealth]{\OPT_\wealth}
\leq 2\Rev[\wealth]{\randomprice}$
for all $\wealth \geq \price$.

% $\quant'$ uniformly from $[0, 1 - F(\price)]$. 
% Then the mechanism post the random per unit price $\price'$ 
% such that $\price' = \price$ with probability $F(\price)$, 
% and $\price' = V(\quant')$ with probability $1-F(\price)$. 
% Note that the ex ante allocation 
% of posting this random price 
% $\price'$ is at most $\quant$. 
% Moreover, when $\price < \price' \leq \wealth$, 
% the revenue of posting price $\price'$ 
% is $\cumprice(\quant')$, 
% and when $\price' > \wealth$, 
% the revenue of posting price $\price'$ 
% is $\wealth \quant'$. 
% Therefore, as shown in \Cref{f:revenue of sample}, 
% the expected revenue of posting this random price 
% is the grey shaded area. 
% Since the revenue curve for the value distribution is regular, 
% this is a 2-approximation to the optimal revenue 
% for every budget $\wealth \geq \price$, i.e., 
% $2\Rev[\wealth]{\price'} \geq 
% \Rev[\wealth]{\OPT}$, 
% and a 2-approximation to the revenue 
% from posting price $\price$ 
% for every budget $\wealth < \price$, i.e., 
% $2\Rev[\wealth]{\price'} \geq 
% \Rev[\wealth]{\price}$.
% Therefore, there exists a quantile 
% $\quant\primed \leq \quant$
% such that $2\Rev[\wealth]{V(\quant\primed)} 
% \geq \Rev[\wealth]{\OPT}$ 
% for $\wealth \geq \price$, 
% and $2\Rev[\wealth]{V(\quant\primed)} 
% \geq \Rev[\wealth]{\price}$ 
% for $\wealth < \price$. 
Thus, there exists some quantile $\quant\primed \leq \quant$ such that
\begin{align*}
\Rev{\EXL} & 
\leq \int_{\lbudget}^{\price} \Rev[\wealth]{\price} dG(\wealth)
+ \int_{\price}^{\hbudget}
\Rev[\wealth]{\OPT_\wealth} dG(\wealth) \\
& \leq \int_{\lbudget}^{\price} 2\Rev[\wealth]{\randomprice} dG(\wealth)
+ \int_{\price}^{\hbudget} 2\Rev[\wealth]{\randomprice} dG(\wealth) 
= 2\cumprice(\quant\primed). 
\qedhere
\end{align*}
\end{proof}

% The high level idea is to relax budget incentive constraint 
% in the optimal ex ante mechanism. 
% For types with budgets smaller than the market clearing price, 
% since the budget binds for those types, 
% we can use the argument in \citet{abr-06} 
% to show that posting the marketing clearing price is 
% a 2-approximation to the optimal ex ante revenue from those types. 
% For types with budgets larger than the market clearing price, 
% if the market clearing price is larger than the Myerson's reserve, 
% the revenue of posting the market clearing price 
% is at least the ex ante revenue from those types. 
% If the market clearing price is smaller than the Myerson's reserve, 
% by applying a random sampling technique, 
% we show that there exists a random price such that the 
% revenue from this random price is a 2-approximation 
% to the optimal revenue from those types without 
% the ex ante constraint. 
% Combining the above results gives us the desired bound. 



% \begin{lemma}
% \label{lem:posting market clearing price for low budget}
% For a single agent 
% with private-budget utility,
% independently distributed value 
% and budget,
% a regular distribution,
% the revenue from 
% posting price 
% $\price = \sfrac{\cumprice(\quant)}{\quant}$
% is a 2-approximation 
% to the optimal ex ante revenue 
% from the types with budget smaller than the 
% market clearing price, 
% i.e., 
% $2\cumprice(\quant) \geq 
% \int_{\lbudget}^{\price} \Rev[\wealth]{\EX} dG(\wealth) $.
% \end{lemma}

% \begin{proof}
% We decompose the optimal ex ante mechanism 
% into $\EXS$ and $\EXL$, 
% where 
% $\Rev[\wealth]{\EX} 
% \leq \Rev[\wealth]{\EXS} 
% + \Rev[\wealth]{\EXL}$. 
% By \Cref{lem:EXS}, we know that 
% $\cumprice(\quant) \geq 
% \expect{\Rev[\wealth]{\EXS}}$. 
% In mechanism $\EXL$, 
% only types with value at least $\price$ 
% will purchase a postive amount of item, 
% and for those types, the budget binds 
% in posting market clearing prices 
% for budget $\wealth \leq \price$. 
% Therefore, the revenue from 
% budget $\wealth \leq \price$ 
% in $\EXL$ is at most the revenue of 
% posting the market clearing price, 
% i.e., 
% $\Rev[\wealth]{\price} \geq \Rev[\wealth]{\EXL}$. 
% Taking the integration, we have 
% $\cumprice(\quant) \geq 
% \int_{\lbudget}^{\price} \Rev[\wealth]{\EXL} dG(\wealth)$. 
% Combining the above results, we have 
% $2\cumprice(\quant) \geq 
% \int_{\lbudget}^{\price} \Rev[\wealth]{\EX} dG(\wealth) $.
% \end{proof}




% \begin{lemma}
% \label{lem:posting market clearing price for high budget}
% For a single agent 
% with private-budget utility,
% independently distributed value 
% and budget,
% a regular distribution,
% if the market clearing price 
% $\price = \sfrac{\cumprice(\quant)}{\quant}$ 
% is larger than the Myerson's reserve, 
% the revenue of posting the 
% market clearing price 
% is at least the optimal ex ante revenue 
% from the types with budget larger than the 
% market clearing price, 
% i.e., 
% $\cumprice(\quant) \geq 
% \int_{\price}^{\hbudget} \Rev[\wealth]{\EX} dG(\wealth)$.
% \end{lemma}
% \begin{proof}
% Consider the optimal ex ante mechanism for 
% types with budget higher than 
% the market clearing price, 
% and we relax the budget constraint for 
% those types. 
% Since the valuation distribution is regular, 
% and the probability the item is sold to 
% those types under market clearing price 
% is at most the ex ante probability $\quant$, 
% the optimal mechanism for those types 
% under ex ante constraint 
% is to post a price $\price'$ 
% at most the market clearing price, 
% which will generate revenue at most 
% $\price' \quant \leq \price \quant = \cumprice(\quant)$. 
% \end{proof}


% %First, in \Cref{lem:public budget optimal under regular}, 
% Next, we state a characterization for the optimal 
% mechanism without ex ante constraint 
% when the budget is public. 
% This characterization will help us upper bound the 
% revenue from budget larger than the market clearing price 
% in \Cref{lem:posting randomized price}. 

% \begin{lemma}[\citealp{LR-96}]
% \label{lem:public budget optimal under regular}
% For a single agent with public-budget utility
% and a regular valuation distribution,
% the revenue optimal mechanism 
% is posting the minimum 
% between her budget and the Myerson reserve.
% \end{lemma}


\begin{figure}[t]
\begin{flushleft}
\hspace{-5pt}
\begin{minipage}[t]{0.48\textwidth}
\centering
\input{Paper/new_result/figure-sample.tex}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\centering
\input{Paper/new_result/figure-sample-small.tex}
\end{minipage}
\end{flushleft}
\caption{\label{f:revenue of sample} 
The grey shaded area is the expected revenue 
of posting the random price defined 
in \Cref{lem:posting randomized price for EXL} 
when the budget is $\wealth$.
The left hand side is the comparison when the budget is large, 
and the right hand side is the comparison when the budget is small. 
}
\end{figure}




% \begin{lemma}
% \label{lem:posting randomized price}
% For a single agent 
% with private-budget utility,
% independently distributed value 
% and budget,
% a regular distribution, 
% if the market clearing price 
% $\price = \sfrac{\cumprice(\quant)}{\quant}$ 
% is smaller than the Myerson's reserve, 
% there exists a random price $\price'$ such that 
% the expected revenue from the random price 
% is a 2-approximation 
% to the optimal revenue 
% from the types with budget larger than the 
% market clearing price, 
% i.e., 
% $2\expect{\Rev[\wealth]{\price'}} \geq 
% \int_{\price}^{\hbudget} \Rev[\wealth]{\OPT} dG(\wealth)$.
% \end{lemma}
% \begin{proof}
% For each budget $\wealth$ larger than the market clearing price, 
% by \Cref{lem:public budget optimal under regular}, 
% the optimal revenue from budget $\wealth$ 
% without ex ante constraint 
% is the revenue of posting price 
% $\min\{\wealth, \myersonReserve\}$.

% Consider the mechanism that draws a random sample 
% $\quant'$ uniformly from $[0, 1 - F(\price)]$. 
% % $\val$ from the value distribution, conditional on the 
% % value being larger than the market clearing price $\price$. 
% Then the mechanism post the random per unit price $\price'$ 
% such that $\price' = \price$ with probability $F(\price)$, 
% and $\price' = V(\quant')$ with probability $1-F(\price)$. 
% Note that the ex ante allocation 
% of posting this random price 
% $\price'$ is at most $\quant$. 
% Moreover, when $\price < \price' \leq \wealth$, 
% the revenue of posting price $\price'$ 
% is $\cumprice(\quant')$, 
% and when $\price' > \wealth$, 
% the revenue of posting price $\price'$ 
% is $\wealth \quant'$. 
% Therefore, as shown in \Cref{f:revenue of sample}, 
% the expected revenue of posting this random price 
% is the grey shaded area. 
% Since the revenue curve for the value distribution is regular, 
% this is a 2-approximation to the optimal revenue 
% for every budget $\wealth \geq \price$, i.e., 
% $2\Rev[\wealth]{\price'} \geq 
% \Rev[\wealth]{\OPT}$.
% Taking integration over the budget 
% gives us the desired bound. 
% \end{proof}



% \begin{proof}[Proof of \Cref{thm: private budget MHR improved}]
% Let $\quant\primed = 
% \argmax_{\quant' \leq \quant} \cumprice(\quant')$.  
% Combining \Cref{lem:posting market clearing price for low budget}, 
% \ref{lem:posting market clearing price for high budget} 
% and \ref{lem:posting randomized price}, 
% we know that 
% \begin{eqnarray*}
% \Rev{\EX} &=& 
% \int_{\lbudget}^{\price} \Rev[\wealth]{\EX} dG(\wealth) 
% + \int_{\price}^{\hbudget} \Rev[\wealth]{\EX} dG(\wealth) \\
% &\leq& 2 \cumprice(\quant) 
% + \max\{\cumprice(\quant), 2\expect{\Rev[\wealth]{\price'}} \} 
% \leq 4 \cumprice(\quant\primed), 
% \end{eqnarray*}
% where $\price'$ is the random price defined 
% in \Cref{lem:posting randomized price}. 
% \end{proof}





% \subsection{Improved Bound}
% In the previous result, 
% we have shown that when the market clearing price 
% is larger than the Myerson's reserve, 
% it is a 3-approximation 
% to the optimal ex ante revenue. 
% In this part, 
% we show that through a decomposition 
% of the per unit prices, 
% we also achieve a 3-approximation 
% when the market clearing price is 
% smaller than the Myerson's reserve. 

% According to \Cref{sec:private}, we decompose 
% the ex ante optimaml mechanism 
% into $\EXS$ and $\EXL$. 
% By \Cref{lem:EXS}, the revenue of $\EXS$ 
% is upper bounded by the revenue of 
% posting the markert clearing price. 
% %$\cumprice(\quant)$. 
% In the following, we will show that 
% under the regularity assumption, 
% the revenue from $\EXL$ can be upper 
% bounded by twice of the optimal price-posting 
% revenue under the ex ante constraint. 

% \begin{lemma}
% \label{lem:posting randomized price for EXL}
% For a single agent 
% with private-budget utility,
% independently distributed value 
% and budget,
% a regular distribution, 
% if the market clearing price 
% $\price = \sfrac{\cumprice(\quant)}{\quant}$ 
% is smaller than the Myerson's reserve, 
% there exists $\quant\primed \leq \quant$
% such that 
% the market clearing revenue from $\quant\primed$
% is a 2-approximation 
% to the revenue from $\EXL$, 
% i.e., 
% $2 \cumprice(\quant\primed) \geq 
% \int_{\lbudget}^{\hbudget} \Rev[\wealth]{\EXL} dG(\wealth)$.
% \end{lemma}
% \begin{proof}
% We decompose the revenue from $\EXL$ by different types. 
% For types with budget smaller than the market clearing price, 
% i.e., $\wealth < \price$, 
% budget binds for those types under market clearing price. 
% Therefore, the revenue for those types from mechanism $\EXL$ 
% is upper bounded by the revenue for those types from 
% posting the market clearing price $\price$. 
% For types with budget larger than the market clearing price, 
% i.e., $\wealth \geq \price$, 
% the revenue from types with budget $\wealth$ is upper bounded by 
% the optimal revenue for budget $\wealth$. 
% Therefore, 
% The revenue for $\EXL$ is upper bounded by 
% \begin{align*}
% \Rev{\EXL} &= 
% \int_{\lbudget}^{\price} \Rev[\wealth]{\EXL} dG(\wealth)
% + \int_{\price}^{\hbudget} \Rev[\wealth]{\EXL} dG(\wealth) \\
% & \leq \int_{\lbudget}^{\price} \Rev[\wealth]{\price} dG(\wealth)
% + \int_{\price}^{\hbudget} \Rev[\wealth]{\OPT} dG(\wealth).
% \end{align*}

% Consider the mechanism that draws a random sample 
% $\quant'$ uniformly from $[0, 1 - F(\price)]$. 
% Then the mechanism post the random per unit price $\price'$ 
% such that $\price' = \price$ with probability $F(\price)$, 
% and $\price' = V(\quant')$ with probability $1-F(\price)$. 
% Note that the ex ante allocation 
% of posting this random price 
% $\price'$ is at most $\quant$. 
% Moreover, when $\price < \price' \leq \wealth$, 
% the revenue of posting price $\price'$ 
% is $\cumprice(\quant')$, 
% and when $\price' > \wealth$, 
% the revenue of posting price $\price'$ 
% is $\wealth \quant'$. 
% Therefore, as shown in \Cref{f:revenue of sample}, 
% the expected revenue of posting this random price 
% is the grey shaded area. 
% Since the revenue curve for the value distribution is regular, 
% this is a 2-approximation to the optimal revenue 
% for every budget $\wealth \geq \price$, i.e., 
% $2\Rev[\wealth]{\price'} \geq 
% \Rev[\wealth]{\OPT}$, 
% and a 2-approximation to the revenue 
% from posting price $\price$ 
% for every budget $\wealth < \price$, i.e., 
% $2\Rev[\wealth]{\price'} \geq 
% \Rev[\wealth]{\price}$.
% Therefore, there exists a quantile 
% $\quant\primed \leq \quant$
% such that $2\Rev[\wealth]{V(\quant\primed)} 
% \geq \Rev[\wealth]{\OPT}$ 
% for $\wealth \geq \price$, 
% and $2\Rev[\wealth]{V(\quant\primed)} 
% \geq \Rev[\wealth]{\price}$ 
% for $\wealth < \price$. 
% Thus, we have 
% \begin{align*}
% \Rev{\EXL} & 
% \leq \int_{\lbudget}^{\price} \Rev[\wealth]{\price} dG(\wealth)
% + \int_{\price}^{\hbudget} \Rev[\wealth]{\OPT} dG(\wealth) \\
% & \leq \int_{\lbudget}^{\price} 2\Rev[\wealth]{V(\quant\primed)} dG(\wealth)
% + \int_{\price}^{\hbudget} 2\Rev[\wealth]{V(\quant\primed)} dG(\wealth) 
% = 2\cumprice(\quant\primed). 
% \qedhere
% \end{align*}
% \end{proof}



==> Paper/new_result/private_budget_mhr.tex <==
\section{Private-budget Utility}

In this section, 
we consider the case where
agents have private-budget utility.
We assume their values and budgets are 
independently distributed,
the valuation distributions
are regular,
and the 
budget distributions
are MHR.
These three assumptions 
guarantee the concavity of 
the price-posting revenue curve,
cf., \Cref{lem:private budget concave price-posting revenue curve}.


\begin{theorem}\label{thm: private budget MHR}
For a single agent 
with private-budget utility, 
assuming 
the value and budget are independently 
distributed,
the valuation distribution is regular
and the budget distribution is MHR,
her price-posting revenue curve $\cumprice$ 
is downward $(\alphaPrivateMHR, \betaPrivateMHR)$-close 
to her ex ante revenue curve $\revcurve$. 
\end{theorem}

Before we give the proof of 
\Cref{thm: private budget MHR},
we list lemmas used in that proof.

\begin{numberedlemma}
{\ref{lem:market clearing price large}}
For a single agent with private-budget utility,
assuming the value and budget are
independently distributed,
and the valuation distribution is regular,
for any ex ante constraint $\quant$,
if the market clearing price $\price$
is at least the Myerson reserve 
$\myersonReserve$,
then at ex ante constraint $\quant$, 
the price-posting revenue 
is a 
$2$-approximation 
to
the ex ante revenue, i.e., 
$2\cumprice(\quant) \geq \revcurve(\quant)$.
\end{numberedlemma}

\begin{numberedlemma}
{\ref{lem:market clearing price small}}
For a single agent with private-budget utility,
assuming the value and budget are
independently distributed,
and the valuation distribution is regular,
for any ex ante constraint $\quant$,
if the market clearing price $\price$
is at most the expected budget 
$\wealth^*$,
then at ex ante constraint $\quant$, 
the price-posting revenue 
is a 
$(2+e)$-approximation 
to
the ex ante revenue, i.e., 
$(2+e)\cumprice(\quant) \geq \revcurve(\quant)$.
\end{numberedlemma}

\begin{lemma}[\citet{LR-96}]
\label{public budget optimal under regular}
Let the valuation distribution $F$ be regular,
and $\myersonReserve$ be the Myerson reserve;
the optimal mechanism for a single agent with 
public budget $\wealth$ is posting 
$\min\{\wealth, \myersonReserve\}$.
\end{lemma}

\begin{lemma}[\citet{CGMW-18}]
\label{lem:post expected budget}
Let $\wealth^*$ be the expectation of an MHR distribution $G$. Let $\mech^*$ be
the optimal mechanism for an 
agent with a public budget $\wealth^*$. 
Then,
assuming the budget and value are independently
distributed,
$\mech^*$ is a $2e$-approximation to the 
optimal revenue when the agent 
has a private budget drawn from $G$.
\end{lemma}

Now we give the proof of \Cref{thm: private budget MHR}.

\begin{proof}[Proof of \Cref{thm: private budget MHR}]
Denote the Myerson reserve by $\myersonReserve$,
and the expected budget by $\wealth^*$. 
Let $\optimalReserve$
be the optimal price for 
the price-posting revenue curve $\cumprice$,
i.e.,
$\optimalReserve = \argmax_\price 
\price\cdot \priceToQuantile(\price, \cumprice)$.
With a budget constraint,
the optimal price $\optimalReserve$
is at most the Myerson reserve $\myersonReserve$.
Since the budget distribution is MHR, 
the expected budget $\wealth^*$
has quantile at least $\sfrac{1}{e}$,
i.e., $\prob{\wealth \geq \wealth^*} 
\geq \sfrac{1}{e}$
(see, e.g., \citet{BM-65}).
Our analysis considers two cases depending on whether
the Myerson reserve is larger or smaller 
than the expected budget.

\paragraph{Prosperous Agent.}
Suppose that the Myerson reserve $\myersonReserve$ 
is smaller than the 
expected budget $\wealth^*$.


Consider any ex ante constraint $\quant$ with 
the market clearing price $\price$
greater than the Myerson reserve $\myersonReserve$.
By \Cref{lem:market clearing price large},
the revenue of posting the 
market clearing price $\price$
is a 2-approximation to 
the $\quant$ ex ante revenue.%, 
%i.e. $\revcurve(\quant) \leq 2\cumprice(\quant)$.

Consider any ex ante constraint $\quant$ with the market
clear price $\price$ 
smaller than  
the Myerson reserve $\myersonReserve$.
Since the valuation distribution is regular and 
the Myerson reserve $\myersonReserve$ 
is smaller than
the expected budget $\wealth^*$,
\Cref{public budget optimal under regular}
shows that
posting the Myerson reserve $\myersonReserve$ 
is the optimal mechanism for an agent with 
public budget $\wealth^*$. 
By \Cref{lem:post expected budget},
its revenue for the agent with private budget,
is a $2e$-approximation to the optimal revenue.
% By the concavity of the post-pricing revenue curve,
% the revenue of posting 
% the market clearing price $\price$
% is at least the revenue
% of posting the Myerson reserve,
% which is an $e$-approximation to the optimal revenue.
% In this case, consider
% posting the Myerson reserve $\myersonReserve$ which 
% achieves a smaller ex ante quantile.
% Since
% the valuation distribution is regular,
% for all types with budget higher 
% than the expected budget $\wealth^*$,
% it extracts the maximum revenue.
% With the fact that
% the expected budget $\wealth^*$ has
% quantile at least $\sfrac{1}{e}$,
% posting the Myerson reserve
% guarantees an $e$-approximation
% to the optimal revenue,
% which is always the upper bound 
% of the $\quant$ ex ante revenue 
% $\revcurve(\quant)$.

\paragraph{Impoverished Agent.} 
Suppose that the Myerson reserve $\myersonReserve$
is larger than the expected budget $\wealth^*$.

Consider any ex ante constraint
$\quant$ with market clearing price 
$\price$ greater than the expected budget $\wealth^*$.
By \cref{lem:market clearing price small},
the revenue of posting the market clearing price $\price$
is a $(2+e)$-approximation to the $\quant$
ex ante revenue, i.e., 
$\revcurve(\quant) \leq (2+e)\cumprice(\quant)$.

Consider any ex ante constraint
$\quant$ with 
the market clearing price $\price$ smaller
than the expected budget $\wealth^*$.
In this case, 
consider posting the expected budget $\wealth^*$
which achieves a smaller ex ante ex ante quantile.
Since the valuation distribution is regular and 
the expected budget $\wealth^*$
is smaller than
the Myerson reserve $\myersonReserve$,
\Cref{public budget optimal under regular}
shows that
posting the expected budget $\wealth^*$ 
is the optimal mechanism for an agent with 
public budget $\wealth^*$. 
By \Cref{lem:post expected budget},
its revenue for the agent with private budget,
is a $2e$-approximation to the optimal revenue.
% Let $\Rev{\OPT(\wealth)}$ be the optimal revenue 
% for types with a fixed budget $\wealth$,
% $\Rev{\OPT}$ be the optimal revenue for all types.,
% and $\Rev{\wealth^*(\wealth)}$ be the mechanism 
% which posts the expected budget $\wealth^*$
% to types with a fixed budget $\wealth$.
% \begin{align*}
%     \Rev{\OPT} &\leq 
%     \int_{\lbudget}^{\wealth^*}
%     \Rev{\OPT(\wealth)}dG(\wealth)
%     +
%     \int_{\wealth^*}^{\hbudget}
%     \Rev{\OPT(\wealth)}dG(\wealth) \\
%     &\leq
%     \int_{\lbudget}^{\wealth^*}
%     \Rev{\OPT(\wealth^*)}dG(\wealth)
%     +
%     \int_{\wealth^*}^{\hbudget}
%     \Rev{\OPT(\wealth)}dG(\wealth) 
% \end{align*}

\bigbreak
\noindent
Collecting all bounds,
for any ex ante constraint $\quant\in[0,1]$,
there exists quantile $\quant\primed$ 
such that 
$\cumprice(\quant\primed) \geq
\frac{1}{2e}\revcurve(\quant)$.
Thus, the price-posting revenue
curve $\cumprice$ is downward
$(\alphaPrivateMHR,\betaPrivateMHR)$-close
to the ex ante revenue curve $\revcurve$.
\end{proof}



==> Paper/new_result/risk_averse.tex <==
\section{Risk Averse Utility}
In this section, 
we consider the case when agents are risk averse. 
Specifically, we consider the risk aversion model 
in \cite{FHH-13}, 
where each agent's utility function has a capacity constraint. 
Given allocation $\alloc$ and 
payment $\price$,
agent's utility with capacity constraint $\capacity$ 
is $\min \{\val\alloc - \price, \capacity\}$. 
We refer to this utility function as \emph{capacitated utility}. 
Moreover, 
following \cite{FHH-13}, in this section, 
we consider the mechanisms 
that are ex-post IR, 
and we requires that losers have no payment, 
and winners pay at most their bids. 
%are ex-post individual rational. 
Next we introduce a definition and two lemmas, 
which is adapted from \cite{FHH-13}. 

% \begin{definition}[\cite{FHH-13}]\label{def:two price}
% A mechanism is a two priced mechanism 
% if when it serves an agent $i$ 
% with quantile $\quant_i$, 
% value $\val_i = \frac{\cumprice_i(\quant_i)}{\quant_i}$, 
% and capacity $\capacity_i$, 
% the payment is either $\val_i$ 
% or $\val_i - \capacity_i$. 
% The probability that agent $i$ is charged with 
% payment $\val_i$ is denoted by $\alloc_{i}^{\val}(\quant_i)$, 
% and the probability that agent $i$ is charged with 
% payment $\val_i - \capacity$ 
% is denoted by $\alloc_{i}^{\capacity}(\quant_i)$. 
% \end{definition}
\begin{definition}[\cite{FHH-13}]\label{def:two price}
A mechanism is a two priced mechanism 
if when it serves an agent 
with quantile $\quant$ 
%value $\val = \frac{\cumprice(\quant)}{\quant}$, 
and capacity $\capacity$, 
the payment is either $\valfunc(\quant)$ 
or $\valfunc(\quant) - \capacity$. 
The probability that agent is charged with 
payment $\valfunc(\quant)$ is denoted by $\alloc^{\val}(\quant)$, 
and the probability that agent is charged with 
payment $\valfunc(\quant) - \capacity$ 
is denoted by $\alloc^{\capacity}(\quant)$. 
\end{definition}

\begin{lemma}[\cite{FHH-13}]\label{lem:two price is opt}
The ex ante optimal mechanism for agents
with capacitated utility is two priced. 
\end{lemma}

% Let $\virt(\val) = \val - \frac{1 - F(\val)}{f(\val)}$
% be Myerson's virtual value function. 
Let $(\cdot)^+ = \max\{\cdot, 0\}$. 
\begin{lemma}[\cite{FHH-13}]\label{lem:upper bound for risk averse}
For any agent with capacity $\capacity$ 
and price-posting revenue cureve $\cumprice$, 
for two priced mechanism with allocation rule 
$\alloc(\quant) = \alloc^{\val}(\quant) 
+ \alloc^{\capacity}(\quant)$, 
the revenue from that agent is 
\begin{equation*}
\Rev{\alloc} \leq 
\expect{(\cumprice'(\quant))^+ \cdot \alloc(\quant)}
+ \expect{(\cumprice'(\quant))^+ 
\cdot \alloc^{\capacity}(\quant)}
+ \expect{\left(\valfunc(\quant)
- \capacity \right)^+ 
\cdot \alloc^{\capacity}(\quant)}
\end{equation*}
\end{lemma}

\begin{theorem}
For a single item environment with an agent 
with maximum value $\maxval$ 
and capacity $\capacity \leq \maxval$, % \geq \max_q \cumprice(q)$, 
if her price-posting revenue curve $\cumprice$ is concave,  
her price-posting revenue curve $\cumprice$ 
is downward $(2 + \ln \frac{\maxval}{\capacity}, 1)$-close 
to her ex ante revenue curve $\revcurve$. 
\end{theorem}
\begin{proof}
For any quantile $\optquant$, 
let $\alloc$ be the optimal allocation 
that satisfies ex-ante allocation constraint $\optquant$. 
By \Cref{lem:upper bound for risk averse}, 
\begin{equation*}
\revcurve(\optquant) = \Rev{\alloc} \leq 
\expect{(\cumprice'(\quant))^+ \cdot \alloc(\quant)}
+ \expect{(\cumprice'(\quant))^+ 
\cdot \alloc^{\capacity}(\quant)}
+ \expect{\left(\valfunc(\quant) 
- \capacity \right)^+ 
\cdot \alloc^{\capacity}(\quant)}
\end{equation*}
Let $\myersonReserve$ be the Myerson's reserve, 
and let 
$\correspondingquant = \min\{
\priceToQuantile(\myersonReserve, \cumprice), \optquant\}$. 
By definition, $\correspondingquant \leq \optquant$. 
Since the price-posting revenue curve is concave, 
posting price 
$\valfunc(\correspondingquant)$
maximizes expected marginal revenue 
under ex ante constraint $\optquant$. 
Therefore, 
$$
\expect{(\cumprice'(\quant))^+ \cdot \alloc(\quant)} 
\leq \cumprice(\correspondingquant)
$$
and 
$$
\expect{(\cumprice'(\quant))^+ 
\cdot \alloc^{\capacity}(\quant)} 
\leq \cumprice(\correspondingquant). 
$$
When $\correspondingquant 
= \priceToQuantile(\myersonReserve, \cumprice)$, 
for any quantile $\quant$, 
$\cumprice(\quant) \leq \cumprice(\correspondingquant)$. 
When $\correspondingquant = \optquant < 
\priceToQuantile(\myersonReserve, \cumprice)$, 
the allocation $\alloc^{\capacity}(\quant)$ 
with ex ante constraint $\optquant$
that maximizes 
$\expect{\left(\valfunc(\quant) 
- \capacity \right)^+ 
\cdot \alloc^{\capacity}(\quant)}$ 
satisfies that 
$\alloc^{\capacity}(\quant) = 1$ 
for $\quant \leq \correspondingquant$,
and $\alloc^{\capacity}(\quant) = 0$
for $\quant > \correspondingquant$. 
Since the price-posting revenue curve is concave, 
in this case, $\cumprice(\quant) \leq \cumprice(\correspondingquant)$ 
when $\quant \leq \correspondingquant$. 
Therefore, 
% Moreover, since the price-posting revenue curve is concave, 
% $\cumprice(\quant) \leq \cumprice(\correspondingquant)$ 
% when $\quant \leq \correspondingquant$, 
% or when $\quant > \correspondingquant$ 
% and $\correspondingquant 
% = \priceToQuantile(\myersonReserve, \cumprice)$. 
% Thus, 
\begin{eqnarray*}
&&\expect{\left(\valfunc(\quant) 
- \capacity \right)^+ 
\cdot \alloc^{\capacity}(\quant)} 
=
\expect{\left(\frac{\cumprice(\quant)}{\quant} 
- \capacity \right)^+ 
\cdot \alloc^{\capacity}(\quant)} 
\leq \expect{\left(\min \left\{\maxval,\frac{
\cumprice(\correspondingquant)}{\quant} \right\} 
- \capacity \right)^+} \\
&=& \int_{\frac{\cumprice(\correspondingquant)}{\maxval}}
^{\min\{1, 
\frac{\cumprice(\correspondingquant)}{\capacity}\}}
\left(\frac{
\cumprice(\correspondingquant)}{\quant} 
- \capacity \right) d\quant
+ \int_{\frac{\cumprice(\correspondingquant)}{\maxval}}^1 
(\maxval - \capacity) dq
\leq \cumprice(\correspondingquant) 
\ln \frac{\maxval}{\capacity}. 
\end{eqnarray*}
Combining the above inequalities, we have
$\revcurve(q) \leq 
\cumprice(\correspondingquant) 
(2 + \ln \frac{\maxval}{\capacity})$.
\end{proof}

When the agent's value distribution is regular, 
her price-posting revenue curve is concave. 

\begin{corollary}
For a single item 
environment where 
each agent $i$ has capacity $\capacity_i$, 
and regular valuation distributions, 
letting $\mincapacity = \min_i (\capacity_i)$ 
be the minimum capacity, 
the approximation factor of
anonymous pricing to the ex ante
relaxation is at most $(2 + \ln \frac{\maxval}{\mincapacity})\rho$. 
\end{corollary}

The following standard example shows that the dependence on 
$\ln \frac{\maxval}{\mincapacity}$ is necessary 
even when there is a single agent. 

\begin{example}\label{exp:single risk agent}
Fix a constant $\maxval$.
Consider a single agent with equal revenue distribution. 
That is, her value $\val$ is 
drawn from $[1, \maxval]$ 
with a density function
$\frac{1}{\val^2}$ for $v \in [1, \maxval)$,
and a mass point of probability $\frac{1}{\maxval}$
on value $\maxval$. 
The revenue for posting any price is $1$. 
Suppose the agent has capacity constraint $\capacity \geq 1$, 
Consider the mechanism that always allocate the item
to the agent, 
and charges her 
$0$ if her value $\val$ is less than $\capacity$, 
and charges her $\val - \capacity$ if 
her value is at least $\capacity$. 
The revenue for this mechanism is 
$\ln \frac{\maxval}{\capacity}$. 
\end{example}

In this section, we require that 
losers have no payment, 
and winners pay at most their bids. 
%the optimal mechanism is ex post IR. 
In the following example, we show that 
price-posting mechanism is not a constant approximation 
to the optimal mechanism
when we allow the winners to pay more than their bids, 
even when the capacity is as large as the support of the value.  

\begin{example}\label{exp:single risk agent with overpay}
Fix a constant $\maxval$.
Consider a single agent with equal revenue distribution as in \Cref{exp:single risk agent}. 
The revenue for posting any price is $1$. 
Suppose the agent has capacity constraint $\capacity = h$, 
Consider the mechanism that always allocate the item
to the agent, 
and charges her 
$v-\maxval$ with probability $\frac{1}{2}$, 
$\maxval$ with probability $\frac{1}{2}$. 
This mechanism is BIC and ex-post IR.  
The revenue for this mechanism is 
half of the welfare, which cannot be 
approximated within a constant fraction by any price-posting mechanism. 
\end{example}

==> Paper/old_result/private_budget.tex <==
\section{Private-budget Utility}
\label{sec:private}
In this section, we consider 
the case where 
agents have private-budget utility.
To obtain a constant approximation bound
for anonymous pricing, 
we assume that 
values and budgets are independently 
distributed,
the valuation distribution
is regular and 
one of two possible assumptions 
on the budget distribution:
(a)
% the expected budget 
% $\wealth^*$ has some 
% constant quantile $\sfrac{1}{\budgetQuantile}$, 
% i.e., $\prob{\wealth \geq \wealth^*} = 
% \sfrac{1}{\budgetQuantile}$;
the probability that the budget
exceeds its expectation is 
at least a constant $\sfrac{1}{\budgetQuantile}$;
and (b)
the budget distribution has \emph{monotone hazard rate (MHR)}, i.e,
$\frac{g(\wealth)}{1-G(\wealth)}$
is monotonically non-decreasing 
with respect to $\wealth$.
Since for a MHR distribution,
a sample exceeds 
its expectation with probability at least 
$\sfrac{1}{e}$
\citep[cf.][]{BM-65},
assumption (b) is special case of 
assumption (a).
% One class of distributions 
% which satisfies the quantile assumption 
% on expected budget with $\budgetQuantile = e$
% is the \emph{monotone hazard rate (MHR)}, i.e,
% $\frac{g(\wealth)}{1-G(\wealth)}$
% is monotonically non-decreasing 
% with respect to $\wealth$
%
% \begin{assumption}\label{asp:value budget independent}
% For each agent $i$, her private value $\vali$
% and private budget $\wealth_i$
% are drawn independently from 
% the valuation distribution
% $F_i$ with support $[0, \hval_i]$
% and 
% the budget distribution 
% $G_i$ with support $[\lbudget_i, \hbudget_i]$ 
% respectively.
% \end{assumption}
% Similar to \Cref{sec:public},
% we drop the index $i$ for agent $i$ for notation simplicity.
% %We use $F$, $f$, $G$, $g$ to 
% %denote the cumulative density function 
% %and 
% %the density function
% %for the valuation distribution $F$ and the
% %budget distribution $G$ respectively.
% \begin{assumption}\label{asp:value regular}
% For each agent, 
% the valuation distribution $F$ is regular.
% \end{assumption}
%
% \renewcommand{\thedefinition}
% {\thesection.\arabic{definition}.A}%
% \begin{assumption}
% \label{asp:expected budget quantile}
% For each agent,
% the expected budget $\wealth^*$. 
% \end{assumption}\addtocounter{definition}{-1}
%
% \renewcommand{\thedefinition}
% {\thesection.\arabic{definition}.B}%
% \begin{assumption}\label{asp:budget MHR}
% For each agent,
% the budget distribution $G$ has 
% \emph{monotone hazard rate (MHR)}, i.e,
% $\frac{g(\wealth)}{1-G(\wealth)}$
% is monotonically non-decreasing 
% with respect to $\wealth$. 
% \end{assumption}
%\Cref{asp:value regular} 
%follows directly from 
%\citet{AHNPY-18} for linear utility model.
We give two examples in Appendix 
\ref{apx:private negative example} which
demonstrate the necessity of these assumptions.
%\Cref{asp:value budget independent},
%\ref{asp:budget MHR}.
%\renewcommand{\thedefinition}
%{\thesection.\arabic{definition}}

\subsection*{Budget Exceeds Expectation with 
Constant Probability}

We first analyze the approximation bound 
for anonymous pricing mechanism
under the assumption that 
the budget exceeds its 
expectation with constant probability 
at least $\sfrac{1}{\budgetQuantile}$.

\begin{theorem}\label{thm:private bound}
A single 
% item 
% environment with 
% an 
agent with private-budget utility
is $(\alphaprivate,\betaprivate)$-regular
if 
value and budget 
are independently distributed,
the valuation distribution is regular,
and the budget exceeds its 
expectation with probability at least
$\sfrac{1}{\budgetQuantile}$.
\end{theorem}

\begin{corollary}
For a single item 
environment with 
agents with private-budget utility,
the worst case
approximation factor of
anonymous pricing to the ex ante
relaxation is at most $\APprivate$
if
values and budgets 
are independently distributed,
the valuation distributions are regular,
and the budgets exceed their 
expectations with probability at least
$\sfrac{1}{\budgetQuantile}$.
\end{corollary}


To prove \Cref{thm:private bound},
it is sufficient to show that 
the private-budget utility under our assumptions 
has price-posting revenue curve 
which is $(\alphaprivate,\betaprivate)$-close for price posting, 
and then apply \Cref{lem:close rev curve imply close pricing}.


We take the following high-level approach which is similar to the
analysis of \citet{abr-06}. Fix any ex ante constraint $\quant$ less
than $\sfrac{1}{(\betaprivate)}$.  Consider the per-unit price induces
ex ante allocation probability exactly $\quant$; henceforth, the {\em
  market clearning price}.  For any allocation and payment
$(\alloc,\price)$ obtained by an agent in the ex ante optimal
mechanism, refer to the agent's per-unit price as $\tilde\price =
\sfrac{\price}{\alloc}$.  We decompose the $\quant$ ex ante optimal
mechanism into two mechanisms where the per-unit price in the first
mechanism for each type is at most the market clearing price, and the
per-unit price in the second mechanism for each type is at least the
market clearing price.  The revenue of the former mechanism is smaller
than the revenue of posting the market clearing price since it sells
less of the item and with a lower per-unit price and, under our
assumptions, the revenue of the latter can be bounded within a
constant factor of the revenue of posting the market clearing price.
The latter analysis considers separately the case of high and low
market clearing prices and in the former derives bounds via the
geometry of revenue curves and in the latter by the assumption on
budgets.
% using the observation that, 
% under our assumption on the budget distribution, 
% either posting the market clearing price is a constant approximation 
% to the optimal revenue even without the budget constraint, 
% or the budget binds in posting the market clearing price 
% for types with budget equal to the expected budget,
% and this induces a lower bound of the revenue 
% in posting the market clearing price.


% Finally, depending on 
% whether the market clearing price is large or small,
% we use two different arguments
% to 
% upper bound the revenue from 
% both decomposed mechanisms 
% by the revenue from 
% posting the market clearing price.
% %We now formalize this plan.

In order to decompose 
the ex ante optimal mechanism,
we first provide a definition
and a characterization 
of all incentive compatible
mechanisms for 
a single agent with private-budget utility,
and her behavior in the mechanisms.

\begin{definition}
An \emph{allocation-payment function} 
$\APF:[0,1] \rightarrow \R_+$
is a mapping from the allocation $\alloc$
purchased by an agent
to the payment $\price$ she is charged.
\end{definition}

\begin{lemma}\label{lem:pricing function characterization}
For a single 
% item environment 
% with a single 
agent 
with private-budget utility,
in any incentive compatible mechanism, %$\mech$,
for all types with any fixed budget,
the mechanism %$\mech$ 
provides 
a convex and non-decreasing allocation-payment function,
%which maps the allocation to the payment, 
and subject to
this allocation-payment function,
each type will purchase as much as she wants 
until the budget constraint binds, 
or the unit-supply constraint binds, or 
the value binds (i.e., her marginal utility
becomes zero).
\end{lemma}
The formal proof of \Cref{lem:pricing function characterization} is
given in \Cref{apx:private}.  At a high level, in private
budget settings, by relaxing the incentive compatiblity constraint for
both values and budgets to the incentive compatiblity constraint only for
values, the payment identity at every fixed budget level is sufficient
to induce an allocation-payment function for all types with that fixed
budget.
% A simple but crucial lemma in our analysis 
% is that subject to a fixed allocation-payment function,
% the revenue from types with higher budget can be upperbounded
% by the revenue from types with lower budget.



% the payment identity induces an allocation-payment function.
% In private-budget utility,  
% the incentive compatible constraints for value 
%  are
% already sufficient to pin down the same payment identity,
% and induce an allocation-payment function 
% for all types with that fixed budget.


Fix an arbitrary ex ante constraint $\quant$ and denoting $\EX$ be the
$\quant$ ex ante optimal mechanism.  Consider the decomposition of
$\EX$ into two mechanisms $\EXS$ and $\EXL$. These decomposed
mechanisms will be incentive compatible for values, but not
necessarily for budgets; a setting we refer to as the
\emph{random-public-budget utility} model.  We require that (a) the
per-unit prices in $\EXS$ for all types are at most the market
clearing price; (b) the allocation for all types in $\EXS$ is at most
the allocation in $\EX$; (c) the per-unit prices in $\EXL$ for all
types are larger than the market clearing price; and (d) the revenue
from $\EX$ (for a private-budgeted agent) is upper bounded by the
revenue from $\EXS$ and $\EXL$ (for a random-public-budgeted agent
with same distribution), i.e., $\Rev{\EX} \leq \Rev{\EXS} +
\Rev{\EXL}$.

The construction is as follows:
For each budget $\wealth$, 
let $\APF_\wealth$ be the allocation-payment function
for types with budget $\wealth$
in mechanism $\EX$, and 
$\alloc^*_\wealth$ be the largest allocation such that
the marginal price is below the market clearing price $p$, i.e.,
$\alloc^*_\wealth =\argmax\{\alloc : \APF_\wealth'(\alloc )\leq p\} $.
Define the allocation-payment functions 
$\APFS_\wealth$ and 
$\APFL_\wealth$ for 
$\EXS$ and $\EXL$ respectively below,
\begin{align*}
    \APFS_\wealth(\alloc) &=
    \left\{
    \begin{array}{ll}
      \APF_\wealth(\alloc)   &   
    \text{if }\alloc \leq \alloc^*_\wealth,\\
        \infty   &  \text{otherwise};
    \end{array}
    \right.
    \quad
    \APFL_\wealth(\alloc) = 
    \left\{
    \begin{array}{ll}
      \APF_\wealth(\alloc^*_\wealth+\alloc) -
      \APF_\wealth(\alloc^*_\wealth)&   
    \text{if }\alloc \leq 1 - \alloc^*_\wealth,\\
        \infty   &  \text{otherwise}.
    \end{array}
    \right.
\end{align*}

\begin{figure}[t]
\begin{flushleft}
\hspace{-5pt}
\begin{minipage}[t]{0.42\textwidth}
\centering
\input{Paper/figure-decomposel.tex}
\end{minipage}
\begin{minipage}[t]{0.57\textwidth}
\centering
\input{Paper/figure-decomposeh.tex}
\end{minipage}
\end{flushleft}
\caption{\label{f:decompose} 
Depicted are allocation-payment function decomposition.
The black lines in both figures are the allocation-payment function 
$\APF_\wealth$ in ex ante optimal mechanism $\EX$; 
the gray dashed lines are the allocation-payment function
$\APFS_\wealth$ 
and
$\APFL_\wealth$ 
in $\EXS$ and $\EXL$, respectively.
}
\end{figure}
In this construction, 
since the original allocation-payment functions
$\APF_\wealth$ in $\EX$
are convex and non-decreasing
for each budget level $\wealth$,
the constructed
allocation-payment functions 
$\APFS_\wealth$ and $\APFL_\wealth$
are also 
convex and non-decreasing.
Hence, for each type,
the payment in $\EX$
is upper bounded by 
the sum of 
the payments in $\EXS$ and $\EXL$,
and 
the requirements above are satisfied.

\begin{lemma}
\label{lem:EXS}
For a single agent with random-public-budget utility,
and independently distributed value and budget, 
for any ex ante constraint $\quant$,
the revenue of $\EXS$ is at most 
the revenue from posting the market clearing price,
i.e., $\cumprice(\quant) \geq \Rev{\EXS}$.
\end{lemma}
\begin{proof}
The ex ante allocation of $\EXS$
is at most the ex ante allocation of $\EX$, 
i.e., $\quant$.
Combining with the fact that the per-unit prices
in $\EXS$ for all types are weakly lower 
than the market clearing price,
its revenue is at most the revenue 
of posting the market clearing price.
\end{proof}

Now, we introduce two lemmas 
\Cref{lem:market clearing price large}
and 
\Cref{lem:market clearing price small}
to upper bound the revenue of 
$\EXL$; the former for the case that the market clearing price is large, and the latter for the case that it is small.
At a high level, 
when the market clearing price is large,
we utilize the 
geometry of revenue curves to bound the revenue;
and 
when the market clearing price is small,
we use the 
assumption on the budget distribution
to bound the revenue.



\begin{lemma}[Large Market Clearing Prices]\label{lem:market clearing price large}
For a single 
% item 
% environment with 
% an
agent with random-public-budget utility,
independently distributed value and budget,
and a regular valuation distribution:
\begin{enumerate}
    \item[(i)] for any ex ante 
    constraint $\quant$
    and market clearing price $\price$
    which is at least the Myerson reserve
    $\myersonReserve$,
    i.e.,
    $\price = 
    \cumprice(\quant)/\quant 
    \geq \myersonReserve$,
    the revenue of posting the market
    clearing price 
    is 
    at least the revenue of $\EXL$, 
    i.e., $\cumprice(\quant) \geq \Rev{\EXL}$;
    \item[(ii)] (otherwise)
    for any ex ante 
    constraint $\quant$
    and market clearing price 
    $\price = 
    \cumprice(\quant)/\quant 
    \geq V(\theta)$ for some $\theta$,
    the revenue of posting the market
    clearing price is an $(\sfrac{1}{(1-\theta)})$-approximation 
    to the revenue of $\EXL$, 
    i.e.,
    $\cumprice(\quant) \geq
    (1-\theta)\cdot \Rev{\EXL}$.
\end{enumerate}
%under \Cref{asp:value budget independent},
%\ref{asp:value regular}, 
% for any ex ante constraint~$\quant$,
% the revenue of posting the market clearing 
% price $\price$
% is an $(\sfrac{1}{(1-\theta)})$-approximation 
% to the revenue of $\EXL$, 
% i.e.,
% $\cumprice(\quant) \geq
% (1-\theta)\cdot \Rev{\EXL}
% $,
% if the market clearing price $\price$
% is at least $V(\theta)$;
% further,
% %the revenue of posting the market clearing 
% %price
% the former
% is at least the 
% latter,
% %revenue of $\EXL$,
% i.e.,
% $\cumprice(\quant) \geq \Rev{\EXL}
% $,
% if the market clearing price $\price$
% is at least the Myerson reserve $\myersonReserve$.
\end{lemma}

Note that the third case,
where the market clearing price is small,
will be handled subsequently by \Cref{lem:market clearing price small}. 

\begin{proof}[Proof of \Cref{lem:market clearing price large}]
In both $\EXL$ and  
the mechanism that posts the market clearing price,
the types with value lower than
the market clearing price 
$\price$ will purchase nothing,
so we only consider the types with value at least $\price$
in this proof. 
Each budget level is considered separately. 
If a $\beta$-approximation is shown separately, 
then $\beta$-approximation holds in combination. 

For types with budget $\wealth \leq \price$, 
by posting the market clearing price $\price$, 
those types always pay their budgets $\wealth$,
which is at least the revenue 
from those types in $\EXL$. 

For types with budget $\wealth > \price$, 
by posting the market clearing price $\price$, 
those types always pay $\price$.
Since the budget constraints do
not bind for these types,
% by 
% posting any price at most
% $\price$,
it is helpful to consider 
the price-posting revenue curve without budget,
which we denote by $\cumpricelinear$.
The regularity of the valuation distribution 
guarantees that
 $\cumpricelinear$ is concave. 
Now we consider two cases: (i)
the market clearing price $\price$ is 
at least the Myerson reserve
$\myersonReserve$;
(ii)
the market clearing price $\price$ is 
less than the Myerson reserve
$\myersonReserve$ but at least
$V(\theta)$.
In both cases, we use the concavity of 
$\cumpricelinear$.

% If the market clearing price 
% $\price$ is at least the
% Myerson reserve $\myersonReserve$,
For case (i),
the concavity of $\cumpricelinear$
implies that higher prices above $\myersonReserve$ 
extracts lower revenue
than $\price$.
Since the per-unit prices in $\EXL$ for all types 
are at least $\price$,
the concavity of $\cumpricelinear$
guarantees that the expected revenue of posting $\price$ 
for types with budget larger than
$p$
is at least the expected revenue for those types in $\EXL$.

For case (ii),
% If the $\price$ is between 
% $\myersonReserve$ and $V(\theta)$,
% the revenue from posting $\price$ is
% at least the revenue from 
% posting $V(\theta)$. 
the concavity of $\cumpricelinear$
implies that lower prices below $\myersonReserve$ 
extracts lower revenue.
Thus, posting $\price$ 
extracts higher revenue than posting  
$V(\theta)$.
Again, the concavity of $\cumpricelinear$
guarantees that 
the revenue of posting  $V(\theta)$ 
is an $(\sfrac{1}{(1-\theta)})$-approximation
to the optimal revenue (i.e., posting 
the Myerson reserve $\myersonReserve$)
generated from these types, 
even with the relaxation of ignoring their budget constraint.

% Therefore, the revenue from posting 
% the market clearing price $\price$ is an $(\sfrac{1}{(1-\theta)})$-approximation
% to $\Rev{\EXL}$ in general, and 
% $2$-approximation if the market clearing price 
% $\price$ is at least 
% the Myerson reserve $\myersonReserve$.

% By posting the market clearing price $\price$, 
% %the market clearing price,
% the types with budget $\wealth \leq \price$ 
% always pay their budget $\wealth$,
% which is at least the revenue from $\EXL$;
% and 
% the types with budget $\wealth > \price$
% always pay $\price$.
% By the assumptions that $\price \geq V(\theta)$
% and valuation distribution is regular, 
% the concavity of the price-posting revenue curve
% guarantees that the revenue from posting 
% the market clearing price is an 
%$(\sfrac{1}{(1-\theta)})$-approximation
% to the optimal revenue without budget constraint.

Combining these bounds above, 
if the market clearing price $\price$
is at least the Myerson reserve
$\myersonReserve$,
then
$
\cumprice(\quant)
\geq
\Rev{\EXL}$;
and otherwise
if the market clearing price $\price$
is at least $V(\theta)$, then
$\cumprice(\quant)
\geq (1 - \theta)\cdot \Rev{\EXL}
$.
\end{proof}

% In the proof of \Cref{lem:market clearing price large},
% we use the assumption 
% that the market clearing price $\price$
% is at least $V(\theta)$ to upper bound the 
% revenue from the types with budget 
% $\wealth$ larger than the 
% market clearing price $\price$.
% By replacing this assumption with a strong assumption
% that %the market clearing price 
% $\price$
% is at least the Myerson reserve $\myersonReserve$,
% a strong result hold with the same argument.

% \begin{corollary}
% \label{cor:market clearing price large Myerson}
% For a single 
% % item 
% % environment with 
% % an
% agent with private-budget utility,
% assuming the value and budget are
% independently distributed,
% and the valuation distribution is regular,
% %under \Cref{asp:value budget independent},
% %\ref{asp:value regular}, 
% for any ex ante constraint $\quant$,
% if the market clearing price $\price$
% is at least the Myerson reserve $\myersonReserve$,
% then the price-posting revenue 
% is a 
% $2$-approximation 
% to
% the ex ante revenue 
% at ex ante constraint $\quant$, i.e., 
% $2\cumprice(\quant) \geq \revcurve(\quant)$.
% \end{corollary}


\begin{lemma}[Small Market Clearing Prices]\label{lem:market clearing price small}
For a single
% item 
% environment with an 
agent with random-public-budget utility,
independently
distributed
 value and budget,
and a budget distribution 
such that 
the budget exceeds its expectation
with probability at least 
$\sfrac{1}{\budgetQuantile}$,
%under \Cref{asp:value budget independent},
%\ref{asp:budget MHR},
for any ex ante constraint $\quant \leq 
%\theta\cdot\budgetQuantile$,
\sfrac{\theta}{\budgetQuantile}$
with market clearing price $\price = \cumprice(\quant)/\quant < V(\theta)$,
the revenue of posting 
the market clearing price $\price$ 
is a 
$(1+\budgetQuantile -
\sfrac{1}{\budgetQuantile})$-approximation to
the revenue of $\EXL$, i.e., 
$(1+\budgetQuantile
-\sfrac{1}{\budgetQuantile}
)\cdot\cumprice(\quant)
\geq \Rev{\EXL}$
\end{lemma}

Before the proof of \Cref{lem:market clearing price small},
we introduce an intermediate lemma used in our argument.

\begin{lemma}\label{lem:decreasing budget}
Fix any convex and 
non-decreasing allocation-payment function,
and any value $\val$,
for any budgets $\wealth\primed$ and
$\wealth\doubleprimed$ such
that $\wealth\primed \leq \wealth\doubleprimed$,
subject to this allocation-payment function,
the payment from the type $(\val, \wealth\primed)$ 
with value $\val$ and budget 
$\wealth\primed$ 
is a 
$(\sfrac{\wealth\doubleprimed}{\wealth\primed})$-approximation
to the payment from the type $(\val, \wealth\doubleprimed)$
with value $\val$ and
budget $\wealth\doubleprimed$.
\end{lemma}
\begin{proof}
% By \Cref{lem:pricing function characterization},
% subject to an allocation-payment function,
% a type will purchase as much as she wants 
% until the budget constraint binds, 
% or the unit-supply constraint binds, or 
% the value binds (i.e., her marginal utility
% becomes zero).

If the type $(\val, \wealth\primed)$ pays
her budget $\wealth\primed$ 
(i.e., the budget constraint binds), 
her payment is a 
$(\sfrac{\wealth\doubleprimed}{\wealth\primed})$-approximation
to the payment from the type $(\val, \wealth\doubleprimed)$,
since the type $(\val, \wealth\doubleprimed)$
pays at most $\wealth\doubleprimed$.

If the type $(\val, \wealth\primed)$ pays less 
than her budget $\wealth$  
(i.e., the unit-supply constraint binds, or 
the value binds),
her allocation is equal to the allocation 
from the type $(\val, \wealth\doubleprimed)$.
Hence, their payments are the same.
\end{proof}


\begin{proof}[Proof of \Cref{lem:market clearing price small}]
Similar to the proof of 
\Cref{lem:market clearing price large},
we only consider the types with value at least $\price$.
Let $\wealth^*$ be the expected budget. 
We claim that all types with 
budget $\wealth^*$ pay their budget
in posting the market clearing price.
Otherwise, 
the unit-demand constraint binds for all
types $(\val,\wealth)$
such that 
$\val \geq \price$,
$\wealth \geq \wealth^*$;
and the assumption that $\price < V(\theta)$
implies
the ex ante allocation for them 
%with budget at least $\wealth^*$
is 
$\prob{\val\geq \price}\cdot\prob{\wealth \geq \wealth^*}
> 
\sfrac{\theta}{\budgetQuantile}$, 
which exceeds the ex ante constraint~$q$, 
a contradiction.


Let $\Rev[\wealth']{\APFL_\wealth}$
be the expected 
revenue of providing the allocation-payment 
function $\APFL_\wealth$ 
in $\EXL$ 
to the types with budget $\wealth'$;
and let $\Rev[\wealth']{\price}$ 
be the expected 
revenue of posting 
the market clearing
price $\price$ 
to the types with budget $\wealth'$.

The following three facts allow 
comparison of
$\Rev{\EXL}$ to 
$\cumprice(\quant)$:
        (a) Posting the market clearing 
        price $\price$
        makes the budget constraints bind 
        for the types
        with budget at most $\wealth^*$, so
        $\RevAPFww \leq \RevPPw$
        for all $\wealth \leq \wealth^*$.
        (b) 
        \Cref{lem:decreasing budget} implies that 
        $\RevAPFww \leq 
        \frac{\wealth}{\wealth^*}
        \RevAPFwEw$
        for all $\wealth \geq \wealth^*$.
        % (c) 
        % Since $\RevPPw$ is weakly increasing in $\wealth$, then
        % $\int_{\lbudget}^{\wealth^*}\RevPPw dG(\wealth)
        % =
        % \cumprice(q) - \int_{\wealth^*}^{\hbudget}\RevPPw dG(\wealth)
        % \leq 
        % \cumprice(q) - \cumprice(q) \cdot \prob{\wealth\geq \wealth^*}
        % =
        % (1-\sfrac{1}{\budgetQuantile})\cumprice(q)$.
        (c) Since 
        the revenue of posting 
        the market clearing price $p$ 
        to an agent with budget $\wealth^*$
        is at most 
        the revenue
        to an agent with budget $\wealth>%$ %higher than
        %$
        \wealth^*$;
        with the assumption that
        budgets exceed the 
        expectation $\wealth^*$ 
        with probability at least 
        $\sfrac{1}{\budgetQuantile}$, 
        it implies that 
        $$
        \RevPPEw\cdot \frac{1}{\budgetQuantile}
        \leq 
        \expect{\RevPPw
        \ \Big| \ 
        \wealth \geq \wealth^*}\cdot
        \prob{\wealth\geq \wealth^*}
        \leq \cumprice(\quant).
        %\qedhere
        $$
We upper bound the revenue of $\EXL$ as follows,
\begin{align*}
        \Rev{\EXL} &=
        \int_{\lbudget}^{\wealth^*} 
        \RevAPFww dG(\wealth) 
        +
        \int_{\wealth^*}^{\hbudget} 
        \RevAPFww dG(\wealth) \\
        &\leq 
        \int_{\lbudget}^{\wealth^*} 
        \RevPPw dG(\wealth)
        +
        \int_{\wealth^*}^{\hbudget} 
        \frac{\wealth}{\wealth^*} 
        \RevAPFwEw dG(\wealth) \\
        &\leq
        (1-\frac{1}{\budgetQuantile})
        \cumprice(\quant)
        +
        \frac{\int_{\wealth^*}^{\hbudget}
        \wealth dG(\wealth)}{\wealth^*} 
        \RevPPEw  \\
        &\leq
        (1-\frac{1}{\budgetQuantile})
        \cumprice(\quant)
        +
        \RevPPEw \leq
        (1+\budgetQuantile-
        \frac{1}{\budgetQuantile})
        \cumprice(\quant)
        \end{align*}
where the first inequality is due to facts (a) and (b); 
in the second inequality, the first term is due to 
$\prob{\wealth \leq \wealth^*} 
\leq 1 - \sfrac{1}{\budgetQuantile}$, 
the revenue $\RevPPw$ is monotone increasing in $\wealth$, 
and by definition $\int_{\lbudget}^{\hbudget} 
        \RevPPw dG(\wealth) = \cumprice(\quant)$, 
%$\RevPPw = \cumprice(\quant)$, 
and the second term is due to fact (a);
and the last inequality is due to fact (c).
\end{proof}

We combine the three lemmas into a proof for
\Cref{thm:private bound}.
\begin{proof}[Proof of \Cref{thm:private bound}]
Set the parameter $\theta = 
\sfrac{\budgetQuantile}{(\budgetQuantile+1)}
% \sfrac{(\budgetQuantile^2-1)}
% {(\budgetQuantile^2 + \budgetQuantile - 1)}
$.
\Cref{lem:EXS}, \Cref{lem:market clearing price large} and 
\Cref{lem:market clearing price small}
implies that for all 
ex ante constraints $\quant \leq
\sfrac{1}{(\budgetQuantile+1)}
% \tfrac{\budgetQuantile^2-1}
% {(\budgetQuantile^2 + \budgetQuantile -
% 1)\budgetQuantile}
$,
the price posting revenue is a 
$(2+\budgetQuantile
%-\sfrac{1}{\budgetQuantile}
)$-approximation 
to the ex ante revenue.
Hence, applying \Cref{lem:close rev curve imply close pricing},
% and \Cref{thm:general AP bound},
% the $(\alphaprivate,\betaprivate)$-close property
% holds and the approximation 
% bound for anonymous pricing 
the result
is proved.
\end{proof}

% \begin{remark}
% Even though in \Cref{thm:private bound}, 
% we assume that the budget distribution is MHR,
% we only use the fact that the quantile of its 
% expectation is at least $\sfrac{1}{e}$ in our proof.
% A similar constant approximation result follows, 
% by replacing this assumption with any constant 
% lower bound guarantee on the expected budget.
% \end{remark}

\subsection*{MHR Budget Distribution}

Assuming that
the value and the budget 
are independently distributed,
the valuation distribution is regular,
and
the budget distribution 
is MHR, 
the price-posting revenue curve is concave. 
This result is formally stated in \Cref{lem:private budget concave price-posting revenue curve}, 
whose proof is deferred to 
Appendix~\ref{apx:private}. 
Due to the concavity of the price-posting revenue curve, 
we show
a better approximation bound 
for anonymous pricing 
using the reduction in \Cref{thm:general EAR bound}. 
% by
% \Cref{thm:general EAR bound}.
% The proof of \Cref{lem:private budget concave price-posting revenue curve}
% %and \Cref{thm: private budget MHR}
% is deferred to 
% Appendix~\ref{apx:private}.


\begin{lemma}\label{lem:private budget concave price-posting revenue curve}
A single
agent with 
private-budget utility 
has a concave price-posting 
revenue curve $\cumprice$ 
if 
her value and budget 
are independently distributed,
the valuation distribution is regular,
and the budget distribution is MHR.
%under \Cref{asp:value budget independent},
%\ref{asp:value regular},
%\ref{asp:budget MHR},
\end{lemma}

% With \Cref{lem:private budget concave price-posting revenue curve}, 
% the price-posting revenue is concave, 
% and we are able to achieve better bounds for 
% MHR budget distributions by applying the approach 
% in \Cref{cor:ex ante close}. 


\begin{theorem}\label{thm: private budget MHR}
A single agent 
with private-budget utility 
has a price-posting revenue curve $\cumprice$ 
that is $\alphaPrivateMHR$-close for ex ante optimization 
to her ex ante revenue curve $\revcurve$, 
if 
her value and budget 
are independently
distributed,
the valuation distribution is regular,
and the budget distribution is MHR. 
\end{theorem}

\begin{corollary}
For a single item 
environment with 
agents with private-budget utility,
the worst case
approximation factor of
anonymous pricing to the ex ante
relaxation is at most $\alphaPrivateMHR\rho$
if values and budgets 
are independently distributed,
the valuation distributions are regular,
and the budget distributions are MHR.
\end{corollary}

Similar to the proof of \Cref{thm:private bound}, 
the idea here is still to decompose the ex ante mechanism and bound them separately. 
To show the closeness property 
for 
ex ante optimization 
rather than
for price-posting,
it is sufficient to 
argue the 
existence of 
good approximation 
at smaller quantile 
for every ex ante constraint.
With the fact 
that 
posting the minimum of 
the expected budget
and the Myerson reserve
guarantees
a relatively good approximation 
to the optimal revenue 
without ex ante constraint,
a better approximation bound for 
anonymous pricing 
can be achieved 
comparing to \Cref{thm:private bound}.

% We achieve a better bound comparing to \Cref{thm:private bound}, 
% because for $\zeta$-close for ex ante relaxation, 
% posting the minimum of the expected budget and the Myerson's reserve 
% guarantees a better approximation ratio 
% when the ex ante constraint is large. 

We first 
list three lemmas used in the proof 
of \Cref{thm: private budget MHR}. 


\begin{lemma}[\citealp{LR-96}]
\label{lem:public budget optimal under regular}
For a single agent with public-budget utility
and a regular valuation distribution,
the revenue optimal mechanism 
is posting the minimum 
between her budget and the Myerson reserve.
\end{lemma}

% \begin{lemma}[\citealp{CGMW-18}]
% \label{lem:post expected budget}
% Let $\mech$ be
% the optimal mechanism for an 
% agent with public-budget utility where
% the budget is $\wealth^*$.
% For a single agent with private-budget utility,
% independently distributed value and budget,
% and a MHR budget distribution
% with expectation $\wealth^*$,
% the revenue of $\mech$
% is a $2e$-approximation to the 
% optimal revenue.
% \end{lemma}

\begin{lemma}
[Posting the Myerson 
Reserve]
\label{lem:posting Myerson reserve}
For a single agent 
with private-budget utility,
independently distributed value 
and budget,
a regular distribution,
and 
a budget distribution
such that the budget exceeds its 
expectation with probability at least
$\sfrac{1}{\budgetQuantile}$,
if the Myerson reserve $\myersonReserve$ is
at most the expected budget $\wealth^*$,
the revenue of posting the Myerson reserve 
$\myersonReserve$ is a 
$\budgetQuantile$-approximation 
to the optimal mechanism.
\end{lemma}
\begin{proof}
Since
the valuation distribution is regular 
and the Myerson reserve
$\myersonReserve$ is at most 
the expected budget $\wealth^*$,
i.e.,
$\myersonReserve \leq \wealth^*$
by posting the Myerson reserve $\myersonReserve$,
for all types with budget at least
the expected budget $\wealth^*$,
it extracts the maximum revenue.
With the assumption that
the budget exceeds
the expected budget $\wealth^*$ with probability
at least 
$\sfrac{1}{\budgetQuantile}$,
posting the Myerson reserve
guarantees an $\budgetQuantile$-approximation
to the optimal revenue.
\end{proof}

\begin{lemma}
[Posting the Expected Budget]
\label{lem:posting expected budget}
For a single agent 
with private-budget utility,
independently distributed value 
and budget,
a regular distribution,
and 
a budget distribution
such that the budget exceeds its 
expectation with probability at least
$\sfrac{1}{\budgetQuantile}$,
if the expected budget $\wealth^*$
is
at most
the Myerson reserve $\myersonReserve$,
the revenue of posting the expected budget 
$\wealth^*$ is a 
$(2\budgetQuantile-1)$-approximation 
to the optimal mechanism.
\end{lemma}
\begin{proof}
Let $\OPT$ be the optimal mechanism;
$\Rev[\wealth]{\OPT}$ be the expected 
revenue 
from types with budget $\wealth$
in the optimal mechanism;
and 
$\Rev[\wealth]{\wealth^*}$
be the expected 
revenue 
from posting 
the expected budget $\wealth^*$ 
to types with budget $\wealth$.
We upper bound the revenue of the optimal 
mechanism 
by considering 
its revenue from types with budget
less than the 
expected budget $\wealth^*$,
and its revenue from types with budget at least
the expected budget $\wealth^*$,
separately.

\paragraph{Types with budget less than the 
expected budget $\wealth^*$}
Condition on the type with budget 
less than 
%the expected budget 
$\wealth^*$,
the revenue in the optimal mechanism 
is at most the revenue 
from posting %the expected budget 
$\wealth^*$ to an agent with public budget 
$\wealth^*$,
i.e.,
$\expect{\Rev[\wealth]{\OPT}\ |\ \wealth<
\wealth^*} \leq 
\Rev[\wealth^*]{\wealth^*}$
Meanwhile,
since the budget exceeds $\wealth^*$
with probability at least 
$\sfrac{1}{\budgetQuantile}$,
posting %the expected budget
$\wealth^*$
to this private-budgeted agent, 
the revenue is a $\budgetQuantile$-approximation
to the revenue from posting %the expected budget 
$\wealth^*$ to an agent with public budget 
$\wealth^*$,
i.e.,
\begin{equation}\label{eq:ub for expected budget rev}
\Rev[\wealth^*]{\wealth^*} \leq 
\budgetQuantile\cdot 
\expect{\Rev[\wealth]{\wealth^*}}.
\end{equation}
Thus, the revenue of posting $\wealth^*$ 
from all types is
a $(\budgetQuantile - 1)$-approximation 
to the revenue from types
with budget less than $\wealth^*$
in the optimal mechanism,
i.e., 
$$
\prob{\wealth< \wealth^*}\cdot \expect{\Rev[\wealth]{\OPT}
\ \Big| \ 
\wealth<
\wealth^*}
\leq 
(1-\sfrac{1}{\budgetQuantile})
\cdot 
\budgetQuantile\cdot 
\expect{\Rev[\wealth]{\wealth^*}}.
$$
 
\paragraph{Types with budget at least the 
expected budget $\wealth^*$}
\Cref{lem:public budget optimal under regular}
implies 
the revenue from types with a fixed budget $\wealth$ 
is at most the revenue of 
posting $\min\{\wealth,\myersonReserve\}$
to them.
Hence,
\begin{align*}
    % \expect{
    % \Rev{\OPT(\wealth)}|\wealth \geq \wealth^*}
    % \cdot
    % \prob{\wealth \geq \wealth^*}
    % &=
    \int_{\wealth^*}^{\hbudget}
    \Rev[\wealth]{\OPT}dG(\wealth)
    &=
    \int_{\wealth^*}^{\hbudget}
    \min\{\wealth,\myersonReserve\}\cdot
    (1 - F(\min\{\wealth,\myersonReserve\}))
    dG(\wealth)
    \\
    &\leq
    \int_{\wealth^*}^{\hbudget}
    \wealth\cdot
    (1 - F(\wealth^*))
    dG(\wealth)
    \leq 
    \wealth^*\cdot 
    (1 - F(\wealth^*))
    %\int_{\lbudget}^{\hbudget}\wealth %dG(\wealth)
    \\
    &=\Rev[\wealth^*]{\wealth^*} \leq 
\budgetQuantile\cdot 
\expect{\Rev[\wealth]{\wealth^*}},
\end{align*}
where the last inequality is due to inequality \eqref{eq:ub for expected budget rev}.
\bigbreak
\noindent
Combine these two bounds above, 
the revenue from posting the expected
budget $\wealth^*$
is a $(2\budgetQuantile-1)$-approximation
to the optimal revenue, i.e.,
$\expect{\Rev[\wealth]{\OPT}} 
\leq 
(2\budgetQuantile-1)\cdot \expect{\Rev[\wealth]{\wealth^*}}
$.\qedhere

% Let $\OPT$ be the optimal mechanism;
% $\Rev{\OPT(\wealth)}$ be the revenue 
% from types with budget $\wealth$
% in the optimal mechanism;
% and 
% $\Rev{\wealth^*(\wealth)}$
% be the revenue 
% from types with budget $\wealth$
% in posting 
% the expected budget $\wealth^*$.
% We upper bound the revenue 
% of the optimal mechanism $\OPT$
% as follows,
% \begin{align*}
%     \Rev{\OPT} &=
%     \expect{
%     \Rev{\OPT(\wealth)}|\wealth \leq \wealth^*}
%     \cdot
%     \prob{\wealth \leq \wealth^*}\\
%     &+
%     \expect{
%     \Rev{\OPT(\wealth)}|\wealth \geq \wealth^*}
%     \cdot
%     \prob{\wealth \geq \wealth^*}
%     \\
%     &\leq
%     \Rev{\wealth^*(\wealth^*)}
%     \cdot (1 - \frac{1}{\budgetQuantile})
% \end{align*}
\end{proof}

Now we give the proof of \Cref{thm: private budget MHR}.

\begin{proof}[Proof of \Cref{thm: private budget MHR}]
Denote the Myerson reserve by $\myersonReserve$,
and the expected budget by $\wealth^*$. 
% Let $\optimalReserve$
% be the optimal price for 
% the price-posting revenue curve $\cumprice$,
% i.e.,
% $\optimalReserve = \argmax_\price 
% \price\cdot \priceToQuantile(\price, \cumprice)$.
% With a budget constraint,
% the optimal price $\optimalReserve$
% is at most the Myerson reserve~$\myersonReserve$.
Since the budget distribution is MHR, 
the probability that the budget exceeds its expectation 
is at least $\sfrac{1}{e}$,
i.e., $\prob{\wealth \geq \wealth^*} 
\geq \sfrac{1}{e}$
(cf., \citet{BM-65}).
Our analysis considers two cases depending on whether
the Myerson reserve 
$\myersonReserve$ is larger or less 
than the expected budget
$\wealth^*$.

\paragraph{Prosperous Agent}
Suppose that the Myerson reserve $\myersonReserve$ 
is less than the 
expected budget~$\wealth^*$.


Consider any ex ante constraint $\quant$ with 
the market clearing price $\price$
larger than the Myerson reserve $\myersonReserve$.
By \Cref{lem:EXS} and \Cref{lem:market clearing price large},
the revenue of posting the 
market clearing price $\price$
is a 2-approximation to 
the $\quant$ ex ante revenue, 
i.e. $\revcurve(\quant) \leq 2\cumprice(\quant)$.

Consider any ex ante constraint 
$\quant$ with the market
clearing price $\price$ 
smaller than  
the Myerson reserve $\myersonReserve$. 
Then the ex ante probability of posting Myerson
reserve
$\myersonReserve$ is at most $\quant$. 
\Cref{lem:posting Myerson reserve}
guarantees that the revenue of posting the
Myerson reserve $\myersonReserve$
is an $e$-approximation to the optimal mechanism.
% Since the valuation distribution is regular and 
% the Myerson reserve $\myersonReserve$ 
% is less than
% the expected budget $\wealth^*$,
% \Cref{public budget optimal under regular}
% shows that
% posting the Myerson reserve $\myersonReserve$ 
% is the optimal mechanism for an agent with 
% public budget $\wealth^*$. 
% By \Cref{lem:post expected budget},
% its revenue for the agent with private budget,
% is a $2e$-approximation to the optimal revenue.
% By the concavity of the post-pricing revenue curve,
% the revenue of posting 
% the market clearing price $\price$
% is at least the revenue
% of posting the Myerson reserve,
% which is an $e$-approximation to the optimal revenue.
% In this case, consider
% posting the Myerson reserve $\myersonReserve$ which 
% achieves a less ex ante quantile.
% Since
% the valuation distribution is regular,
% for all types with budget higher 
% than the expected budget $\wealth^*$,
% it extracts the maximum revenue.
% With the fact that
% the expected budget $\wealth^*$ has
% quantile at least $\sfrac{1}{e}$,
% posting the Myerson reserve
% guarantees an $e$-approximation
% to the optimal revenue,
% which is always the upper bound 
% of the $\quant$ ex ante revenue 
% $\revcurve(\quant)$.

\paragraph{Impoverished Agent} 
Suppose that the Myerson reserve $\myersonReserve$
is larger than the expected budget $\wealth^*$.

Consider any ex ante constraint
$\quant$ with market clearing price 
$\price$ larger than the expected budget $\wealth^*$.
By \Cref{lem:EXS} and \Cref{lem:market clearing price small},
the revenue of posting the market clearing price $\price$
is a $(2+e-\sfrac{1}{e})$-approximation to the $\quant$
ex ante revenue, i.e., 
$\revcurve(\quant) \leq (2+e-\sfrac{1}{e})\cumprice(\quant)$.

Consider any ex ante constraint
$\quant$ with 
the market clearing price $\price$ smaller
than the expected budget $\wealth^*$.
In this case, 
posting the expected budget $\wealth^*$
achieves a smaller ex ante allocation.
\Cref{lem:posting expected budget} % reserve}
guarantees that the revenue of posting the
expected budget $\wealth^*$
is a $(2e-1)$-approximation to the optimal mechanism.
% Since the valuation distribution is regular and 
% the expected budget $\wealth^*$
% is less than
% the Myerson reserve $\myersonReserve$,
% \Cref{public budget optimal under regular}
% shows that
% posting the expected budget $\wealth^*$ 
% is the optimal mechanism for an agent with 
% public budget $\wealth^*$. 
% By \Cref{lem:post expected budget},
% its revenue for the agent with private budget,
% is a $2e$-approximation to the optimal revenue.
% Let $\Rev{\OPT(\wealth)}$ be the optimal revenue 
% for types with a fixed budget $\wealth$,
% $\Rev{\OPT}$ be the optimal revenue for all types.,
% and $\Rev{\wealth^*(\wealth)}$ be the mechanism 
% which posts the expected budget $\wealth^*$
% to types with a fixed budget $\wealth$.
% \begin{align*}
%     \Rev{\OPT} &\leq 
%     \int_{\lbudget}^{\wealth^*}
%     \Rev{\OPT(\wealth)}dG(\wealth)
%     +
%     \int_{\wealth^*}^{\hbudget}
%     \Rev{\OPT(\wealth)}dG(\wealth) \\
%     &\leq
%     \int_{\lbudget}^{\wealth^*}
%     \Rev{\OPT(\wealth^*)}dG(\wealth)
%     +
%     \int_{\wealth^*}^{\hbudget}
%     \Rev{\OPT(\wealth)}dG(\wealth) 
% \end{align*}

\bigbreak
\noindent
Collecting all bounds,
for any ex ante constraint $\quant\in[0,1]$,
there exists quantile $\quant\primed\leq \quant$ 
such that 
$\cumprice(\quant\primed) \geq
(\sfrac{1}{(2e-1)})\cdot \revcurve(\quant)$.
Thus, the price-posting revenue
curve $\cumprice$ is 
$\alphaPrivateMHR$-close 
for ex ante optimization 
to the ex ante revenue curve $\revcurve$.
\end{proof}


==> Paper/old_result/reduction-framework.tex <==
\section{A General Reduction Framework}
\label{sec:framework}
In this section, we introduce 
two different reduction approaches 
for analyzing the approximation ratio of the anonymous pricing mechanism
in the setting where the agents may not have linear utility.
In the general case, 
when the price-posting revenue curve is not concave, 
we define a ``closeness'' condition 
between the price-posting revenue curve 
and the ex ante revenue curve, 
that guarantees constant  
approximation for anonymous pricing mechanism. 
In some situations where
the price-posting revenue curve is concave, 
we show that a weaker condition 
is sufficient to guarantee the same approximation factor. 
The flow of our reduction framework is shown in \Cref{f:framework}. 
The key idea in our approach is that 
the ex ante revenue is given mathematically by $\{\revcurve_i\}_{i=1}^n$; 
and the revenue of anonymous pricing is given by $\{\cumprice_i\}_{i=1}^n$. 
For linear utility, regularity implies they are equal. 
Thus, we can have a reduction from the non-linear utility 
to the linear utility 
to analyze the approximation ratio of anonymous pricing. 

\begin{figure}[t]
\centering
\input{Paper/figure-reduction.tex}
\caption{\label{f:framework} 
The reduction framework.
}
\end{figure}

\begin{definition}
\label{def:general regularity}
An agent's price-posting revenue curve $\cumprice$
\emph{$(\alpha, \beta)$-approximates}
his ex ante revenue curve $\revcurve$ at an
effective-price 
$\exanteprice$, 
if $\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice) 
\geq \frac{1}{\beta} 
\priceToQuantile(\exanteprice, \revcurve)$.
We call the agent 
\emph{$(\alpha, \beta)$-regular}
if this condition holds at all $\exanteprice$. 
We define $(1,1)$-regular as regular. 
%Moreover, $(1,1)$-regular is regular. 
% An agent satisfies 
% $(\alpha, \beta)$-approximating anonymous pricing property 
% at price $\exanteprice$, 
% if let 
%     $\exanteprobability=
%     \argmax\{\quant:\quant \cdot \exanteprice 
%     = \revcurve(\quant)\}$
%     and  
%     $\correspondingquant=
%     \argmax\{\quant:\quant\cdot \frac{\exanteprice}{\alpha}
%     = \cumprice(\quant)\}$,
%     then 
%     $\correspondingquant \geq \frac{\exanteprobability}{\beta}$. 
\end{definition}



% Before we give the formal result about the connection between
% the 
% $(\alpha, \beta)$-approximating 
% anonymous pricing property 
% and 
% the approximation bound for anonymous pricing,
It is instructive to see some examples  
under the linear utility assumption.
%(e.g., linear utility, 
%risk-averse utility under prospect theory model).


\begin{example}
Given the valuation distribution
is regular,
agents with linear utility function 
is $(1, 1)$-regular.
The anonymous pricing is a
$\rho$-approximation to 
the ex ante relaxation.
\end{example}

\begin{example}
Given the valuation distribution
is arbitrary (possibly irregular),
agents with linear utility function 
is $(\infty, \infty)$-regular.
The anonymous pricing is an
$n$-approximation 
to the ex ante relaxation
where $n$ is the number of agents.
\end{example}

\begin{comment}
\begin{example}
Given the valuation distribution 
is regular,
the weighting function is constant-bounded,
the risk-averse utility under
prospect theory model
(cf., \citet{CGMP-18})
satisfies $(\infty, \infty)$-approximating anonymous pricing property.
The approximation from anonymous pricing 
to the ex ante relaxation 
is a super constant.
\end{example}
\end{comment}


% \begin{definition}
% For any instance $\instance = (\agents, \typespace, \distributions, \util)$, 
% define its reduced instance as 
% $\linearinstance = (\agents, \lineartypespace, \lineardistributions, \linearutil)$, 
% where $\linearutil$ represents the linear utility function. 
% Moreover, for any agent~$i$, 
% the price-posting revenue curve of agent $i$ in the reduced instance is equal to her ex ante revenue curve in the original instance. 
% That is, $\postlinearcurve_i(\quant) = \revcurve_i(\quant)$ for all agent $i$ and for all quantile~$\quant$. 
% \end{definition}

\begin{theorem}\label{thm:general AP bound}
Given agents with 
ex ante revenue 
curves 
$\{\revcurve_i\}_{i=1}^n$
and price-posting revenue curves
$\{\cumprice_i\}_{i=1}^n$,
if the revenue of posting effective price $\exanteprice$ 
on revenue curve $\{\revcurve_i\}_{i=1}^n$
is a 
$\linearapproxratio$-approximation to the ex ante relaxation
revenue of those agents, 
i.e., 
$\pricerev(
\{\revcurve_i\}_{i=1}^n, \exanteprice) 
\geq \frac{1}{\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$, 
and for any agent $i$, 
the price-posting revenue curve $\cumprice_i$ 
$(\alpha, \beta)$-approximates the ex ante 
revenue curve $\revcurve_i$ at $\exanteprice$, 
then
posting anonymous price 
$\sfrac{\exanteprice}{\alpha}$
is an $(\alpha\beta\gamma)$-approximation
to the ex ante relaxation, 
i.e.,
$\pricerev(\{\cumprice_i\}_{i=1}^n, 
\frac{\exanteprice}{\alpha})
\geq \frac{1}{\alpha \beta 
\linearapproxratio}
\exanterev(\{\revcurve_i\}_{i=1}^n)$. 
\end{theorem}
\begin{proof}
By our assumption, 
the quantile of agent $i$ for posting price $\frac{\exanteprice}{\alpha}$ is 
$\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i) 
\geq \frac{1}{\beta}
\priceToQuantile(\exanteprice, \revcurve_i)$. 
Therefore, the revenue of posting price $\frac{\exanteprice}{\alpha}$ in the original instance is 
\begin{eqnarray*}
    \pricerev(\{\cumprice_i\}_{i=1}^n,
    \frac{\exanteprice}{\alpha}) 
    &=& \frac{\exanteprice}{\alpha} \cdot 
    \left(1 - \prod\nolimits_i (1-\priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice_i)) \right) 
    \geq \frac{\exanteprice}{\alpha} \cdot 
    \left(1 - \prod\nolimits_i (1 - \frac{1}{\beta}
    \priceToQuantile(\exanteprice, \revcurve_i)) \right) \\
    &\geq& \frac{\exanteprice}{\alpha\beta} \cdot \left(1 - \prod\nolimits_i 
    (1 - \priceToQuantile(\exanteprice, \revcurve_i)) \right) 
    = \frac{1}{\alpha\beta}
    \pricerev(\{\revcurve_i\}_{i=1}^n, \exanteprice) \\
    &\geq&\frac{1}{\alpha \beta \linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n). \qedhere
\end{eqnarray*}
\end{proof}

At a high level, 
the assumption 
$\pricerev(
\{\revcurve_i\}_{i=1}^n, \exanteprice) 
\geq \frac{1}{\linearapproxratio} \exanterev(\{\revcurve_i\}_{i=1}^n)$
can be interpreted as
a reduction to the 
anonymous price-posting 
approximation for linear utility agents. 
By \Cref{lem:ex-ante is concave}, the ex ante revenue curve is concave and thus,
by \Cref{thm:linear bound}, 
the 
approximation ratio $\gamma$
is
at most 
$\rho \approx e$.


\begin{corollary}
%For the single item environment, 
If agents are $(\alpha, \beta)$-regular, 
the worst case approximation factor of 
anonymous pricing to the ex ante relaxation 
is
$\alpha \beta \rho$.
\end{corollary}


Next we provide a sufficient condition for agents to be
$(\alpha, \beta)$-regular.

\begin{definition}
The agent's price-posting revenue curve $\cumprice$ 
is \emph{$(\alpha, \beta)$-close for price posting} 
to her ex ante revenue curve $\revcurve$, 
if 
$\cumprice(\quant) \geq \frac{1}{\alpha} \revcurve(\quant)$ 
for all
$\quant \in [0, 1/\beta]$. 
\end{definition}


\begin{figure}[t]
\begin{flushleft}
\hspace{-5pt}
\begin{minipage}[t]{0.49\textwidth}
\centering
\setlength{\unitlength}{1cm}
\thinlines
\input{Paper/figure-regular}
\end{minipage}
\begin{minipage}[t]{0.49\textwidth}
\input{Paper/figure-close}
\end{minipage}
\end{flushleft}
\vspace{-10pt}
\caption{\label{f:definition} 
The left hand side illustrates an example that 
the price-posting revenue curve $\cumprice$ is 
$(\alpha, \beta)$-regular, i.e., $\correspondingquant = \priceToQuantile(\exanteprice/\alpha, \cumprice) \geq \sfrac{\exanteprobability}{\beta}$.  
The right hand side illustrates an example that 
the price-posting revenue curve $\cumprice$ is 
$(\alpha, \beta)$-close for price posting
to ex ante revenue curve $\revcurve$, i.e., $\cumprice(\quant) \geq \revcurve(\quant)/\alpha$ for $\quant \in [0,\sfrac{1}{\beta}]$.
}
\end{figure}


\begin{lemma}\label{lem:close rev curve imply close pricing}
If an agent's price-posting revenue curve $\cumprice$ 
is $(\alpha, \beta)$-close for price posting 
to her ex ante revenue curve $\revcurve$, 
then she is $(\alpha, \beta)$-regular. 
\end{lemma}
\begin{proof}
For any price $\exanteprice$, 
let the per-unit price 
$\correspondingprice = \frac{\exanteprice}{\alpha}$. 
Let $\exanteprobability
= \priceToQuantile(\exanteprice, \revcurve)$
and  
$\correspondingquant
= \priceToQuantile(\frac{\exanteprice}{\alpha}, \cumprice)$. 
If the quantile $\exanteprobability \leq \frac{1}{\beta}$, 
since $\cumprice$ is $(\alpha, \beta)$-close for price posting to $\revcurve$, 
$\cumprice(\exanteprobability) \geq \frac{1}{\alpha} \revcurve(\exanteprobability)$. 
Therefore, 
$\frac{\exanteprice \cdot \exanteprobability}{\alpha}
\leq \cumprice(\exanteprobability)$, 
which implies $\correspondingquant \geq \exanteprobability$. 

If $\exanteprobability > \frac{1}{\beta}$, 
and if $\correspondingquant \geq \frac{1}{\beta}$, 
then Lemma \ref{lem:close rev curve imply close pricing} holds. 
If $\correspondingquant < \frac{1}{\beta}$, 
then $\revcurve(\correspondingquant) 
\leq \alpha \cumprice(\correspondingquant)$. 
Therefore, $\exanteprice \cdot \correspondingquant %= \alpha \correspondingprice \cdot \correspondingquant 
\geq \revcurve(\correspondingquant)$, 
which contradicts to the assumption that 
$\exanteprobability > \frac{1}{\beta} \geq \correspondingquant$. 
\end{proof}



% \begin{figure}[t]
% \centering
% \input{Paper/close_imply_regular.tex}
% \caption{\label{f:close_imply_regular} 
% The thick curve is the ex ante revenue curve $\revcurve$ for the agent, 
% and the thin curve is the ex ante revenue curve $\revcurve$
% shrunk by a factor of $\alpha$. 
% The dashed curve is the price-posting revenue curve $\cumprice$ for the agent. 
% Note that any price only crosses the revenue curve 
% at most once other than the point $(0,0)$. 
% From the figure, we know that the quantile 
% $\correspondingquant$
% of posting price $\sfrac{\exanteprice}{\alpha}$ 
% in revenue curve $\cumprice$ is at least 
% the quantile 
% $\exanteprobability$
% of posting effective price $\exanteprice$ 
% in revenue curve $\revcurve$. 
% }
% \end{figure}

Next we give a reduction framework that enables simpler and stronger
approximation bounds when the price-posting revenue curve is concave.
This framework takes the lower path in \Cref{f:framework} and is
easier to prove because the analysis compares ex ante optimal
mechanisms with revenue curves $\cumprice$ and $\revcurve$ rather than
comparing anonymous pricing with these revenue curves.

\begin{definition}
The agent's price-posting revenue curve $\cumprice$ 
is \emph{$\zeta$-close for ex ante optimization} 
to her ex ante revenue curve $\revcurve$, 
if for all $\quant \in [0, 1]$, 
there exists a quantile 
$\correspondingquant \leq \quant$ such that 
$\cumprice(\correspondingquant) \geq \frac{1}{\zeta} \revcurve(\quant)$. 
\end{definition}

Note that $(\alpha, \beta)$-regular implies $\alpha\beta$-close for ex
ante optimization.  Furthermore, $(1,1)$-regularity, $(1,1)$-closeness for
posted pricing, and $1$-closeness for ex ante optimization are all
equivalent.  

\begin{theorem}
\label{thm:general EAR bound}
Given agents with 
ex ante revenue 
curves 
$\{\revcurve_i\}_{i=1}^n$
and price-posting revenue curves
$\{\cumprice_i\}_{i=1}^n$,
if for each agent $i$, 
her price-posting revenue curve $\cumprice_i$
is $\zeta$-close for ex ante optimization
to her ex ante revenue curve $\revcurve_i$, 
then
the optimal ex ante relaxation on revenue curves 
$\{\cumprice_i\}_{i=1}^n$ 
is a $\zeta$-approximation
to the optimal ex ante relaxation on revenue curves 
$\{\revcurve_i\}_{i=1}^n$,  
i.e.,
$\exanterev(\{\cumprice_i\}_{i=1}^n)
\geq \frac{1}{\zeta}
\exanterev(\{\revcurve_i\}_{i=1}^n)$. 
\end{theorem}
\begin{proof}
Let $\quant_i$ be the optimal ex ante relaxation for 
ex ante revenue curves 
$\{\revcurve_i\}_{i=1}^n$, 
%and let $\quant'_i = \min\{\quant_i, \frac{1}{\beta}\}$. 
%By \Cref{lem:ex-ante is concave}, the ex ante revenue curve is concave. 
%We know that $\revcurve_i(\quant'_i) 
%\geq \frac{1}{\beta} \revcurve_i (\quant_i)$. 
%Moreover, 
and let~$\correspondingquant_i$ be the corresponding quantile 
such that 
$\correspondingquant_i \leq \quant'_i$ 
and $\cumprice_i(\correspondingquant_i) 
\geq \frac{1}{\zeta}\revcurve(\quant'_i)$. 
We have 
\begin{equation*}
    \exanterev(\{\cumprice_i\}_{i=1}^n) 
    \geq \sum\nolimits_i \cumprice_i(\correspondingquant_i) 
    \geq \frac{1}{\zeta}\, \sum\nolimits_i \revcurve(\quant_i) 
    = \frac{1}{\zeta}\, \exanterev(\{\revcurve_i\}_{i=1}^n). \qedhere
\end{equation*}
\end{proof}

\begin{corollary}\label{cor:ex ante close}
%For the single item environment, 
If for each agent $i$, 
her price-posting revenue curve $\cumprice_i$
is concave, 
and is $\zeta$-close for ex ante optimization 
to her ex ante revenue curve $\revcurve_i$, 
then 
the worst case approximation factor of 
anonymous pricing to the ex ante relaxation 
is
$\zeta \rho$.
\end{corollary}

Our regularity and closeness definitions are monotone.  With this
observation, our framework can be applied to environments with heterogeneous
utility functions.  For example, suppose some of the agents have
private budget constraints and some of the agents are risk averse.  If
each agent $i \in \{1,\ldots,n\}$ is $(\alpha_i, \beta_i)$-regular then anonymous pricing for
these agents is a $(\max\{\alpha_i\} \cdot \max\{\beta_i\} \cdot
\rho)$-approximation to the optimal ex ante relaxation.


\begin{lemma}\label{lem:closeness is downward imply}
For any $\alpha' \geq \alpha \geq 1$, $\beta' \geq \beta \geq 1$, and
$\zeta' \geq \zeta \geq 1$; $(\alpha, \beta)$-regularity implies
$(\alpha', \beta')$-regularity, $(\alpha, \beta)$-closeness for price posting
implies $(\alpha', \beta')$-closeness for price posting, and $\zeta$-closeness
for ex ante optimization implies $\zeta'$-close for ex ante optimization.
\end{lemma}



% \begin{itemize}
%     \item $(\alpha, \beta)$-regular implies $(\alpha', \beta')$-regular; 

%     \item 
%     $(\alpha, \beta)$-close for price posting 
%     implies $(\alpha', \beta')$-close for price posting;
    
%     \item 
%     $\zeta$-close for ex ante relaxation 
%     implies $\zeta'$-close for ex ante relaxation.
% \end{itemize}






